The iron and oxygen content of LMC Classical Cepheids and its implications for the Extragalactic Distance Scale and Hubble constant

Classical Cepheids are primary distance indicators and a crucial stepping stone to determining the present-day Hubble constant Ho to the precision and accuracy required to constrain apparent deviations from the LCDM Concordance Cosmological Model. We have measured the iron and oxygen abundances of of 89 Cepheids in the LMC, one of the anchors of the local Distance Scale, quadrupling the prior sample and including 68 of the 70 Cepheids used to constrain Ho by the SH0ES program. The goal is to constrain the extent to which the Cepheid luminosity is influenced by their chemical composition, an important contributor to the uncertainty on the determination of the Ho itself and a critical factor in the internal consistency of the distance ladder. We have derived stellar parameters and abundances from a self-consistent spectroscopic analysis based on Equivalent Width of absorption lines. The [Fe/H] distribution of LMC Cepheids is a single Gaussian with a mean of -0.4079+-0.003 dex (0.1 dex systematic uncertainty) and sigma 0.076+-0.003 dex. The latter is fully compatible with the measurement error and supports the low dispersion of 0.069 mag seen in the NIR HST LMC period-luminosity relation. The uniformity of the abundance has the important consequence that the LMC Cepheids alone cannot provide any meaningful constraint on the dependence of the Cepheid Period-Luminosity relation on chemical composition at any wavelength. This revises a prior claim based on a small sample of 22 LMC Cepheids that there was little dependence (or uncertainty) between composition and NIR luminosity, a conclusion which would produce a conflict between anchors of the distance ladder with different mean abundance. The chemical homogeneity of the LMC Cepheid population makes it an ideal environment to calibrate the metallicity dependence between the more metal poor SMC and metal rich Milky Way and NGC4258.

==> SH0ES LMC spectroscopy(1)/Tables/linelist/linelist.tex <==
4892.86 & FeI & -0.876 & 4.22 \\
4893.81 & FeII & -4.157 & 2.83 \\
4917.23 & FeI & -1.160 & 4.19 \\
4923.92 & FeII & -1.559 & 2.89 \\
4924.77 & FeI & -2.114 & 2.28 \\
4932.08 & FeI & -1.483 & 4.65 \\
4950.10 & FeI & -1.500 & 3.42 \\
4973.10 & FeI & -0.690 & 3.96 \\
4993.35 & FeII & -3.684 & 2.81 \\
4994.13 & FeI & -3.080 & 0.92 \\
5029.62 & FeI & -2.000 & 3.42 \\
5044.21 & FeI & -2.017 & 2.85 \\
5049.82 & FeI & -1.355 & 2.28 \\
5054.64 & FeI & -1.921 & 3.64 \\
5056.84 & FeI & -1.940 & 4.26 \\
5067.15 & FeI & -0.484 & 4.22 \\
5072.67 & FeI & -0.834 & 4.22 \\
5083.34 & FeI & -2.958 & 0.96 \\
5090.77 & FeI & -0.440 & 4.26 \\
5100.65 & FeII & -4.222 & 2.81 \\
5126.19 & FeI & -1.060 & 4.26 \\
5132.67 & FeII & -6.427 & 6.73 \\
5133.69 & FeI & 0.360 & 4.18 \\
5171.60 & FeI & -1.793 & 1.49 \\
5197.58 & FeII & -3.575 & 12.89 \\
5198.71 & FeI & -2.135 & 2.22 \\
5215.18 & FeI & -0.860 & 3.27 \\
5216.27 & FeI & -2.150 & 1.61 \\
5217.39 & FeI & -1.070 & 3.21 \\
5234.62 & FeII & -2.138 & 3.22 \\
5242.49 & FeI & -0.967 & 3.63 \\
5243.78 & FeI & -1.120 & 4.26 \\
5256.93 & FeII & -4.327 & 2.89 \\
5257.65 & FeI & -2.753 & 3.57 \\
5281.79 & FeI & -0.834 & 3.04 \\
5288.53 & FeI & -1.490 & 3.69 \\
5307.36 & FeI & -2.987 & 1.61 \\
5324.18 & FeI & -0.110 & 3.21 \\
5325.55 & FeII & -3.185 & 3.22 \\
5326.14 & FeI & -2.071 & 3.57 \\
5339.93 & FeI & -0.630 & 3.27 \\
5362.86 & FeII & -2.616 & 3.20 \\
5364.87 & FeI & 0.228 & 4.45 \\
5365.40 & FeI & -1.020 & 3.57 \\
5367.47 & FeI & 0.443 & 4.42 \\
5373.71 & FeI & -0.710 & 4.47 \\
5379.57 & FeI & -1.514 & 3.69 \\
5383.37 & FeI & 0.645 & 4.31 \\
5389.49 & FeI & -7.973 & 5.33 \\
5391.46 & FeI & -0.777 & 4.15 \\
5393.17 & FeI & -0.720 & 3.24 \\
5398.28 & FeI & -0.710 & 4.45 \\
5405.77 & FeI & -1.844 & 0.99 \\
5410.91 & FeI & 0.398 & 4.47 \\
5414.07 & FeII & -3.644 & 3.22 \\
5415.20 & FeI & 0.642 & 4.39 \\
5417.04 & FeI & -1.660 & 4.42 \\
5424.07 & FeI & 0.778 & 4.32 \\
5425.25 & FeII & -3.352 & 3.20 \\
5434.52 & FeI & -2.122 & 1.01 \\
5445.04 & FeI & 0.211 & 4.39 \\
5452.09 & FeI & -2.812 & 3.64 \\
5464.28 & FeI & -1.400 & 4.14 \\
5466.40 & FeI & -0.285 & 4.37 \\
5497.52 & FeI & -2.849 & 1.01 \\
5501.47 & FeI & -3.047 & 0.96 \\
5506.78 & FeI & -2.797 & 0.99 \\
5522.45 & FeI & -1.520 & 4.21 \\
5531.98 & FeI & -1.600 & 4.91 \\
5534.84 & FeII & -2.865 & 3.25 \\
5543.15 & FeI & -4.651 & 3.69 \\
5554.89 & FeI & -0.270 & 4.55 \\
5560.21 & FeI & -1.160 & 4.43 \\
5561.24 & FeI & -1.204 & 4.61 \\
5562.70 & FeI & -0.642 & 4.43 \\
5565.70 & FeI & -0.214 & 4.61 \\
5572.84 & FeI & -0.280 & 3.40 \\
5576.09 & FeI & -0.940 & 3.43 \\
5584.76 & FeI & -2.270 & 3.57 \\
5586.77 & FeI & -2.903 & 4.26 \\
5627.49 & FeII & -4.062 & 3.39 \\
5633.95 & FeI & -0.320 & 4.99 \\
5635.85 & FeI & -9.120 & 5.37 \\
5638.26 & FeI & -0.720 & 4.22 \\
5641.43 & FeI & -1.150 & 4.26 \\
5653.86 & FeI & -1.610 & 4.39 \\
5658.82 & FeI & -0.760 & 3.40 \\
5661.34 & FeI & -1.756 & 4.28 \\
5679.02 & FeI & -0.900 & 4.65 \\
5686.53 & FeI & -0.446 & 4.55 \\
5691.50 & FeI & -1.490 & 4.30 \\
5707.05 & FeI & -2.350 & 3.64 \\
5717.83 & FeI & -0.960 & 4.28 \\
5720.89 & FeI & -1.632 & 4.55 \\
5731.76 & FeI & -1.270 & 4.26 \\
5834.02 & FeI & -0.979 & 4.91 \\
5835.10 & FeI & -2.040 & 4.26 \\
5838.37 & FeI & -2.290 & 3.94 \\
5848.13 & FeI & -1.057 & 4.61 \\
5849.68 & FeI & -2.633 & 3.69 \\
5852.21 & FeI & -5.954 & 5.62 \\
5853.15 & FeI & -4.254 & 1.49 \\
5855.07 & FeI & -1.478 & 4.61 \\
5856.09 & FeI & -1.328 & 4.29 \\
5858.78 & FeI & -2.349 & 4.22 \\
5859.59 & FeI & -0.418 & 4.55 \\
5861.11 & FeI & -2.268 & 4.28 \\
5862.36 & FeI & -0.125 & 4.55 \\
5873.21 & FeI & -2.109 & 4.26 \\
5877.79 & FeI & -2.233 & 4.18 \\
5883.82 & FeI & -1.310 & 3.96 \\
5885.05 & FeI & -1.479 & 4.99 \\
5902.47 & FeI & -1.313 & 4.59 \\
5902.55 & FeI & -2.695 & 5.87 \\
5905.67 & FeI & -0.770 & 4.65 \\
5916.25 & FeI & -2.994 & 2.45 \\
5921.26 & FeI & -0.685 & 4.65 \\
5927.79 & FeI & -1.070 & 4.65 \\
5929.68 & FeI & -1.380 & 4.55 \\
5930.18 & FeI & -0.057 & 4.65 \\
5934.65 & FeI & -1.120 & 3.93 \\
5940.99 & FeI & -1.638 & 4.18 \\
5943.58 & FeI & -4.192 & 2.20 \\
5956.69 & FeI & -4.608 & 0.86 \\
5959.91 & FeI & -2.496 & 4.14 \\
5975.35 & FeI & -0.693 & 4.83 \\
5976.78 & FeI & -1.236 & 3.94 \\
5983.68 & FeI & -0.485 & 4.55 \\
5984.81 & FeI & -0.198 & 4.73 \\
5987.06 & FeI & -0.432 & 4.79 \\
5991.37 & FeII & -3.647 & 3.15 \\
6003.01 & FeI & -1.100 & 3.88 \\
6003.02 & FeI & -6.715 & 5.51 \\
6007.96 & FeI & -0.597 & 4.65 \\
6008.56 & FeI & -0.980 & 3.88 \\
6008.56 & FeI & -7.961 & 2.95 \\
6020.17 & FeI & -0.125 & 4.61 \\
6024.06 & FeI & 0.223 & 4.55 \\
6027.05 & FeI & -1.089 & 4.08 \\
6041.47 & FeI & -1.500 & 5.01 \\
6045.47 & FeII & -2.413 & 6.21 \\
6055.40 & FeI & -1.479 & 4.96 \\
6056.00 & FeI & -0.320 & 4.73 \\
6062.85 & FeI & -3.798 & 2.18 \\
6063.31 & FeI & -0.862 & 4.91 \\
6065.48 & FeI & -1.530 & 2.61 \\
6078.49 & FeI & -0.323 & 4.79 \\
6079.01 & FeI & -1.100 & 4.65 \\
6082.71 & FeI & -3.573 & 2.22 \\
6084.10 & FeII & -3.854 & 3.20 \\
6085.26 & FeI & -2.710 & 2.76 \\
6089.59 & FeI & -3.616 & 4.58 \\
6093.64 & FeI & -1.470 & 4.61 \\
6094.37 & FeI & -1.920 & 4.65 \\
6096.66 & FeI & -1.880 & 3.98 \\
6127.91 & FeI & -1.400 & 4.14 \\
6136.61 & FeI & -1.400 & 2.45 \\
6136.99 & FeI & -2.950 & 2.20 \\
6137.69 & FeI & -1.403 & 2.59 \\
6141.02 & FeII & -5.128 & 3.23 \\
6149.25 & FeII & -2.732 & 3.89 \\
6151.62 & FeI & -3.299 & 2.18 \\
6156.37 & FeI & -3.274 & 3.40 \\
6165.36 & FeI & -1.474 & 4.14 \\
6170.51 & FeI & -0.475 & 4.79 \\
6173.33 & FeI & -2.880 & 2.22 \\
6173.34 & FeI & -4.244 & 5.33 \\
6179.39 & FeII & -2.599 & 5.57 \\
6180.20 & FeI & -2.650 & 2.73 \\
6183.56 & FeI & -1.175 & 5.03 \\
6185.69 & FeI & -0.730 & 5.65 \\
6187.99 & FeI & -1.670 & 3.94 \\
6200.31 & FeI & -2.437 & 2.61 \\
6213.43 & FeI & -2.480 & 2.22 \\
6215.14 & FeI & -1.320 & 4.19 \\
6219.28 & FeI & -2.433 & 2.20 \\
6220.78 & FeI & -2.068 & 3.88 \\
6221.67 & FeI & -5.971 & 0.86 \\
6226.73 & FeI & -1.965 & 3.88 \\
6229.23 & FeI & -2.810 & 2.85 \\
6230.72 & FeI & -1.281 & 2.56 \\
6232.66 & FeI & -5.049 & 5.01 \\
6238.39 & FeII & -2.637 & 3.89 \\
6239.36 & FeII & -4.731 & 2.81 \\
6240.31 & FeI & -1.917 & 4.14 \\
6240.65 & FeI & -3.170 & 2.22 \\
6246.32 & FeI & -0.770 & 3.60 \\
6247.56 & FeII & -2.340 & 3.89 \\
6252.56 & FeI & -1.687 & 2.40 \\
6253.83 & FeI & -1.300 & 4.73 \\
6261.53 & FeI & -0.929 & 5.06 \\
6265.13 & FeI & -2.550 & 2.18 \\
6269.96 & FeII & -4.613 & 3.25 \\
6270.22 & FeI & -2.610 & 2.86 \\
6286.13 & FeI & -0.670 & 5.62 \\
6297.79 & FeI & -2.740 & 2.22 \\
6300.30 & OI & -9.776 & 0.00 \\
6301.50 & FeI & -0.710 & 3.65 \\
6302.49 & FeI & -0.968 & 3.69 \\
6307.52 & FeII & -5.417 & 2.83 \\
6311.50 & FeI & -3.141 & 2.83 \\
6315.81 & FeI & -1.630 & 4.08 \\
6322.69 & FeI & -2.426 & 2.59 \\
6330.85 & FeI & -1.720 & 4.73 \\
6335.33 & FeI & -2.177 & 2.20 \\
6336.82 & FeI & -0.850 & 3.69 \\
6338.88 & FeI & -1.040 & 4.79 \\
6344.15 & FeI & -2.923 & 2.43 \\
6355.03 & FeI & -2.291 & 2.85 \\
6358.70 & FeI & -4.468 & 0.86 \\
6363.78 & OI & -10.258 & 0.02 \\
6369.46 & FeII & -4.291 & 2.89 \\
6380.74 & FeI & -1.376 & 4.19 \\
6383.73 & FeII & -2.275 & 5.55 \\
6385.46 & FeII & -2.663 & 5.55 \\
6392.54 & FeI & -4.526 & 2.28 \\
6393.60 & FeI & -1.580 & 2.43 \\
6400.00 & FeI & -0.270 & 3.60 \\
6400.32 & FeI & -4.318 & 0.92 \\


==> SH0ES LMC spectroscopy(1)/Tables/linelist/linelist10.tex <==
4892.86 & FeI & -0.876 & 4.22 \\
4893.81 & FeII & -4.157 & 2.83 \\
4917.23 & FeI & -1.160 & 4.19 \\
4923.92 & FeII & -1.559 & 2.89 \\
4924.77 & FeI & -2.114 & 2.28 \\
4932.08 & FeI & -1.483 & 4.65 \\
4950.10 & FeI & -1.500 & 3.42 \\
4973.10 & FeI & -0.690 & 3.96 \\
4993.35 & FeII & -3.684 & 2.81 \\
4994.13 & FeI & -3.080 & 0.92 \\
\ldots & \ldots & \ldots & \ldots \\ 


==> SH0ES LMC spectroscopy(1)/Tables/obslog/obslog.tex <==
OGLE0434 & 2020-11-07T02:47:44.709 & 59160.11649 \\ 
OGLE0434 & 2020-11-07T02:47:52.206 & 59160.11658 \\ 
OGLE0501 & 2020-10-24T04:50:05.197 & 59146.20145 \\ 
OGLE0501 & 2020-10-24T04:50:13.252 & 59146.20154 \\ 
OGLE0512 & 2020-10-24T05:25:26.486 & 59146.22600 \\ 
OGLE0512 & 2020-10-24T05:25:36.488 & 59146.22612 \\ 
OGLE0528 & 2020-10-09T07:28:41.908 & 59131.31160 \\ 
OGLE0528 & 2020-10-09T07:28:48.852 & 59131.31168 \\ 
OGLE0545 & 2020-11-07T03:00:20.624 & 59160.12524 \\ 
OGLE0545 & 2020-11-07T03:00:29.841 & 59160.12535 \\ 
OGLE0590 & 2020-10-26T08:19:13.387 & 59148.34668 \\ 
OGLE0590 & 2020-10-26T08:19:21.279 & 59148.34677 \\ 
OGLE0594 & 2020-10-24T06:09:42.936 & 59146.25675 \\ 
OGLE0594 & 2020-10-24T06:09:49.913 & 59146.25683 \\ 
OGLE0594 & 2020-10-24T06:37:41.388 & 59146.27617 \\ 
OGLE0594 & 2020-10-24T06:37:49.106 & 59146.27626 \\ 
OGLE0648 & 2020-11-07T03:29:44.538 & 59160.14565 \\ 
OGLE0648 & 2020-11-07T03:29:52.365 & 59160.14574 \\ 
OGLE0683 & 2020-11-07T04:07:52.232 & 59160.17213 \\ 
OGLE0683 & 2020-11-07T04:07:59.591 & 59160.17222 \\ 
OGLE0712 & 2020-11-07T04:40:03.399 & 59160.19448 \\ 
OGLE0712 & 2020-11-07T04:40:11.101 & 59160.19457 \\ 
OGLE0716 & 2020-11-09T02:55:21.519 & 59162.12178 \\ 
OGLE0716 & 2020-11-09T02:55:29.431 & 59162.12187 \\ 
OGLE0727 & 2020-11-10T02:20:29.106 & 59163.09756 \\ 
OGLE0727 & 2020-11-10T02:20:36.899 & 59163.09765 \\ 
OGLE0757 & 2020-11-08T07:39:04.532 & 59161.31880 \\ 
OGLE0757 & 2020-11-08T07:39:11.448 & 59161.31888 \\ 
OGLE0757 & 2020-11-08T08:04:12.210 & 59161.33625 \\ 
OGLE0757 & 2020-11-08T08:04:20.535 & 59161.33635 \\ 
OGLE0770 & 2020-11-10T02:46:39.776 & 59163.11574 \\ 
OGLE0770 & 2020-11-10T02:46:47.380 & 59163.11583 \\ 
OGLE0787 & 2020-11-10T06:01:33.654 & 59163.25108 \\ 
OGLE0787 & 2020-11-10T06:01:41.419 & 59163.25117 \\ 
OGLE0798 & 2020-11-09T03:45:06.506 & 59162.15633 \\ 
OGLE0798 & 2020-11-09T03:45:14.930 & 59162.15642 \\ 
OGLE0800 & 2020-11-10T06:29:41.506 & 59163.27062 \\ 
OGLE0800 & 2020-11-10T06:29:48.611 & 59163.27070 \\ 
OGLE0812 & 2020-11-10T07:03:07.455 & 59163.29384 \\ 
OGLE0812 & 2020-11-10T07:03:15.545 & 59163.29393 \\ 
OGLE0819 & 2020-11-10T07:43:40.739 & 59163.32200 \\ 
OGLE0819 & 2020-11-10T07:43:52.080 & 59163.32213 \\ 
OGLE0821 & 2020-11-11T03:48:03.727 & 59164.15838 \\ 
OGLE0821 & 2020-11-11T03:48:12.083 & 59164.15847 \\ 
OGLE0831 & 2020-11-11T04:07:18.368 & 59164.17174 \\ 
OGLE0831 & 2020-11-11T04:07:29.223 & 59164.17187 \\ 
OGLE0844 & 2020-11-11T04:50:47.006 & 59164.20193 \\ 
OGLE0844 & 2020-11-11T04:50:53.984 & 59164.20201 \\ 
OGLE0847 & 2020-11-11T05:15:54.805 & 59164.21938 \\ 
OGLE0847 & 2020-11-11T05:16:01.798 & 59164.21947 \\ 
OGLE0848 & 2020-11-10T08:09:36.138 & 59163.34000 \\ 
OGLE0848 & 2020-11-10T08:09:44.729 & 59163.34010 \\ 
OGLE0888 & 2020-11-09T07:56:53.314 & 59162.33117 \\ 
OGLE0888 & 2020-11-09T07:57:01.486 & 59162.33127 \\ 
OGLE0915 & 2020-11-11T05:49:47.683 & 59164.24291 \\ 
OGLE0915 & 2020-11-11T05:49:54.803 & 59164.24300 \\ 
OGLE0915 & 2020-11-11T06:14:14.760 & 59164.25989 \\ 
OGLE0915 & 2020-11-11T06:14:23.954 & 59164.26000 \\ 
OGLE0936 & 2020-11-11T06:45:04.374 & 59164.28130 \\ 
OGLE0936 & 2020-11-11T06:45:11.371 & 59164.28138 \\ 
OGLE0949 & 2020-11-12T04:02:31.627 & 59165.16842 \\ 
OGLE0949 & 2020-11-12T04:02:39.350 & 59165.16851 \\ 
OGLE0966 & 2020-10-09T06:54:12.669 & 59131.28765 \\ 
OGLE0966 & 2020-10-09T06:54:20.033 & 59131.28773 \\ 
OGLE0969 & 2020-11-11T07:33:38.138 & 59164.31502 \\ 
OGLE0969 & 2020-11-11T07:33:45.430 & 59164.31511 \\ 
OGLE0970 & 2020-11-12T04:37:44.057 & 59165.19287 \\ 
OGLE0970 & 2020-11-12T04:37:51.994 & 59165.19296 \\ 
OGLE0975 & 2020-11-12T05:07:49.280 & 59165.21376 \\ 
OGLE0975 & 2020-11-12T05:07:56.657 & 59165.21385 \\ 
OGLE0978 & 2020-11-12T05:43:29.440 & 59165.23854 \\ 
OGLE0978 & 2020-11-12T05:43:36.373 & 59165.23862 \\ 
OGLE0986 & 2020-11-11T08:11:38.521 & 59164.34142 \\ 
OGLE0986 & 2020-11-11T08:11:47.349 & 59164.34152 \\ 
OGLE0992 & 2020-10-09T07:06:01.942 & 59131.29586 \\ 
OGLE0992 & 2020-10-09T07:06:10.051 & 59131.29595 \\ 
OGLE1001 & 2020-10-09T07:50:15.613 & 59131.32657 \\ 
OGLE1001 & 2020-10-09T07:50:23.258 & 59131.32666 \\ 
OGLE1031 & 2020-10-10T07:28:59.547 & 59132.31180 \\ 
OGLE1031 & 2020-10-10T07:29:06.498 & 59132.31188 \\ 
OGLE1058 & 2020-11-12T06:27:15.380 & 59165.26893 \\ 
OGLE1058 & 2020-11-12T06:27:23.256 & 59165.26902 \\ 
OGLE1080 & 2020-11-12T06:43:42.249 & 59165.28035 \\ 
OGLE1080 & 2020-11-12T06:43:49.212 & 59165.28043 \\ 
OGLE1109 & 2020-11-12T07:09:59.799 & 59165.29861 \\ 
OGLE1109 & 2020-11-12T07:10:08.313 & 59165.29871 \\ 
OGLE1112 & 2020-10-09T08:13:59.599 & 59131.34305 \\ 
OGLE1112 & 2020-10-09T08:14:06.556 & 59131.34313 \\ 
OGLE1313 & 2020-11-13T05:21:20.693 & 59166.22316 \\ 
OGLE1313 & 2020-11-13T05:21:29.103 & 59166.22325 \\ 
OGLE1313 & 2020-11-13T05:45:49.390 & 59166.24015 \\ 
OGLE1313 & 2020-11-13T05:45:58.204 & 59166.24026 \\ 
OGLE1374 & 2020-11-13T06:16:19.724 & 59166.26134 \\ 
OGLE1374 & 2020-11-13T06:16:27.869 & 59166.26143 \\ 
OGLE1374 & 2020-11-13T06:47:09.528 & 59166.28275 \\ 
OGLE1374 & 2020-11-13T06:47:17.066 & 59166.28284 \\ 
OGLE1389 & 2020-11-12T07:43:34.177 & 59165.32192 \\ 
OGLE1389 & 2020-11-12T07:43:45.198 & 59165.32205 \\ 
OGLE1411 & 2020-11-14T04:31:15.249 & 59167.18837 \\ 
OGLE1411 & 2020-11-14T04:31:22.186 & 59167.18845 \\ 
OGLE1411 & 2020-11-14T05:00:24.541 & 59167.20862 \\ 
OGLE1411 & 2020-11-14T05:00:31.543 & 59167.20870 \\ 
OGLE1417 & 2020-11-14T05:36:07.841 & 59167.23342 \\ 
OGLE1417 & 2020-11-14T05:36:18.216 & 59167.23354 \\ 
OGLE1424 & 2020-11-15T06:27:35.742 & 59168.26916 \\ 
OGLE1424 & 2020-11-15T06:27:44.466 & 59168.26926 \\ 
OGLE1424 & 2020-11-15T07:07:14.905 & 59168.29670 \\ 
OGLE1424 & 2020-11-15T07:07:23.692 & 59168.29680 \\ 
OGLE1431 & 2020-11-13T07:22:36.098 & 59166.30736 \\ 
OGLE1431 & 2020-11-13T07:22:43.839 & 59166.30745 \\ 
OGLE1463 & 2020-11-16T04:10:21.074 & 59169.17386 \\ 
OGLE1463 & 2020-11-16T04:10:29.399 & 59169.17395 \\ 
OGLE1463 & 2020-11-16T04:34:10.830 & 59169.19040 \\ 
OGLE1463 & 2020-11-16T04:34:18.574 & 59169.19049 \\ 
OGLE1466 & 2020-11-14T06:23:13.022 & 59167.26612 \\ 
OGLE1466 & 2020-11-14T06:23:19.965 & 59167.26620 \\ 
OGLE1466 & 2020-11-14T07:00:02.432 & 59167.29169 \\ 
OGLE1466 & 2020-11-14T07:00:09.425 & 59167.29178 \\ 
OGLE1490 & 2020-11-17T06:06:55.941 & 59170.25481 \\ 
OGLE1490 & 2020-11-17T06:07:04.005 & 59170.25491 \\ 
OGLE1526 & 2020-11-17T06:48:23.576 & 59170.28361 \\ 
OGLE1526 & 2020-11-17T06:48:31.776 & 59170.28370 \\ 
OGLE1526 & 2020-11-17T07:13:23.492 & 59170.30097 \\ 
OGLE1526 & 2020-11-17T07:13:31.015 & 59170.30105 \\ 
OGLE1539 & 2020-11-17T07:44:06.925 & 59170.32230 \\ 
OGLE1539 & 2020-11-17T07:44:13.896 & 59170.32238 \\ 
OGLE1578 & 2020-11-07T07:53:38.353 & 59160.32892 \\ 
OGLE1578 & 2020-11-07T07:53:45.281 & 59160.32900 \\ 
OGLE1587 & 2020-11-13T08:04:53.644 & 59166.33673 \\ 
OGLE1587 & 2020-11-13T08:05:01.362 & 59166.33682 \\ 
OGLE1616 & 2020-11-15T07:51:39.184 & 59168.32754 \\ 
OGLE1616 & 2020-11-15T07:51:46.194 & 59168.32762 \\ 
OGLE1637 & 2020-10-24T05:11:10.930 & 59146.21610 \\ 
OGLE1637 & 2020-10-24T05:11:19.585 & 59146.21620 \\ 
OGLE1641 & 2020-10-24T05:44:00.477 & 59146.23889 \\ 
OGLE1641 & 2020-10-24T05:44:08.585 & 59146.23899 \\ 
OGLE1647 & 2020-11-14T07:41:41.998 & 59167.32062 \\ 
OGLE1647 & 2020-11-14T07:41:49.422 & 59167.32071 \\ 
OGLE1677 & 2020-11-08T07:18:16.489 & 59161.30436 \\ 
OGLE1677 & 2020-11-08T07:18:24.568 & 59161.30445 \\ 
OGLE1862 & 2020-11-09T06:22:31.686 & 59162.26564 \\ 
OGLE1862 & 2020-11-09T06:22:39.818 & 59162.26574 \\ 
OGLE1939 & 2020-11-07T06:40:06.347 & 59160.27785 \\ 
OGLE1939 & 2020-11-07T06:40:14.688 & 59160.27795 \\ 
OGLE1939 & 2020-11-07T07:14:17.266 & 59160.30159 \\ 
OGLE1939 & 2020-11-07T07:14:24.209 & 59160.30167 \\ 
OGLE1941 & 2020-11-07T05:17:10.861 & 59160.22026 \\ 
OGLE1941 & 2020-11-07T05:17:18.460 & 59160.22035 \\ 
OGLE1941 & 2020-11-07T05:55:57.686 & 59160.24720 \\ 
OGLE1941 & 2020-11-07T05:56:07.369 & 59160.24731 \\ 
OGLE1994 & 2020-11-10T03:46:29.223 & 59163.15728 \\ 
OGLE1994 & 2020-11-10T03:46:36.577 & 59163.15737 \\ 
OGLE2012 & 2020-11-09T07:07:02.917 & 59162.29656 \\ 
OGLE2012 & 2020-11-09T07:07:09.787 & 59162.29664 \\ 
OGLE2019 & 2020-11-10T04:26:44.718 & 59163.18524 \\ 
OGLE2019 & 2020-11-10T04:26:51.980 & 59163.18532 \\ 
OGLE2043 & 2020-11-10T04:46:01.060 & 59163.19862 \\ 
OGLE2043 & 2020-11-10T04:46:09.062 & 59163.19872 \\ 
OGLE2043 & 2020-11-10T05:11:39.588 & 59163.21643 \\ 
OGLE2043 & 2020-11-10T05:11:48.170 & 59163.21653 \\ 
\hline
OGLE0510 & 2000-10-11T04:34:30.713 & 51828.19063 \\ 
OGLE0510 & 2000-10-11T04:44:53.443 & 51828.19784 \\ 


==> SH0ES LMC spectroscopy(1)/Tables/obslog/obslog10.tex <==
OGLE0434 & 2020-11-07T02:47:44.709 & 59160.11649 \\ 
OGLE0434 & 2020-11-07T02:47:52.206 & 59160.11658 \\ 
OGLE0501 & 2020-10-24T04:50:05.197 & 59146.20145 \\ 
OGLE0501 & 2020-10-24T04:50:13.252 & 59146.20154 \\ 
OGLE0512 & 2020-10-24T05:25:26.486 & 59146.22600 \\ 
OGLE0512 & 2020-10-24T05:25:36.488 & 59146.22612 \\ 
OGLE0528 & 2020-10-09T07:28:41.908 & 59131.31160 \\ 
OGLE0528 & 2020-10-09T07:28:48.852 & 59131.31168 \\ 
OGLE0545 & 2020-11-07T03:00:20.624 & 59160.12524 \\ 
OGLE0545 & 2020-11-07T03:00:29.841 & 59160.12535 \\ 
\ldots & \ldots & \ldots \\ 
\hline
OGLE0510 & 2000-10-11T04:34:30.713 & 51828.19063 \\ 
OGLE0510 & 2000-10-11T04:44:53.443 & 51828.19784 \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abus/Fe_abundances.tex <==
OGLE0434 & -0.40 & 0.12 & 0.07 & 101 & -0.43 & 0.13 & 0.04 & 15 \\ 
OGLE0501 & -0.42 & 0.09 & 0.05 & 84 & -0.43 & 0.06 & 0.03 & 12 \\ 
OGLE0510 & -0.38 & 0.11 & 0.03 & 82 & -0.39 & 0.14 & 0.03 & 9 \\ 
OGLE0512 & -0.48 & 0.13 & 0.06 & 91 & -0.41 & 0.11 & 0.01 & 14 \\ 
OGLE0528 & -0.41 & 0.12 & 0.04 & 91 & -0.43 & 0.07 & 0.02 & 15 \\ 
OGLE0545 & -0.37 & 0.09 & 0.06 & 78 & -0.40 & 0.04 & 0.05 & 10 \\ 
OGLE0590 & -0.41 & 0.10 & 0.23 & 83 & -0.38 & 0.13 & 0.08 & 15 \\ 
OGLE0594 & -0.49 & 0.14 & 0.12 & 71 & -0.50 & 0.02 & 0.10 & 6 \\ 
OGLE0648 & -0.45 & 0.09 & 0.06 & 98 & -0.47 & 0.09 & 0.04 & 17 \\ 
OGLE0683 & -0.38 & 0.11 & 0.07 & 90 & -0.40 & 0.14 & 0.05 & 16 \\ 
OGLE0712 & -0.33 & 0.11 & 0.05 & 101 & -0.34 & 0.11 & 0.05 & 16 \\ 
OGLE0716 & -0.45 & 0.09 & 0.05 & 100 & -0.45 & 0.08 & 0.05 & 14 \\ 
OGLE0727 & -0.55 & 0.09 & 0.17 & 70 & -0.58 & 0.10 & 0.17 & 13 \\ 
OGLE0757 & -0.35 & 0.08 & 0.06 & 75 & -0.34 & 0.11 & 0.05 & 14 \\ 
OGLE0770 & -0.44 & 0.10 & 0.04 & 96 & -0.45 & 0.05 & 0.03 & 14 \\ 
OGLE0787 & -0.38 & 0.16 & 0.05 & 63 & -0.37 & 0.07 & 0.06 & 8 \\ 
OGLE0798 & -0.41 & 0.10 & 0.06 & 82 & -0.45 & 0.08 & 0.05 & 12 \\ 
OGLE0800 & -0.57 & 0.10 & 0.10 & 88 & -0.49 & 0.19 & 0.04 & 15 \\ 
OGLE0812 & -0.39 & 0.11 & 0.07 & 98 & -0.40 & 0.16 & 0.06 & 18 \\ 
OGLE0819 & -0.29 & 0.11 & 0.03 & 85 & -0.29 & 0.06 & 0.02 & 11 \\ 
OGLE0821 & -0.58 & 0.10 & 0.06 & 88 & -0.56 & 0.10 & 0.01 & 14 \\ 
OGLE0831 & -0.40 & 0.10 & 0.05 & 88 & -0.44 & 0.06 & 0.04 & 12 \\ 
OGLE0844 & -0.34 & 0.11 & 0.08 & 82 & -0.33 & 0.12 & 0.07 & 12 \\ 
OGLE0847 & -0.40 & 0.12 & 0.05 & 89 & -0.44 & 0.08 & 0.02 & 14 \\ 
OGLE0848 & -0.46 & 0.08 & 0.10 & 65 & -0.46 & 0.06 & 0.07 & 9 \\ 
OGLE0888 & -0.41 & 0.10 & 0.06 & 100 & -0.45 & 0.12 & 0.04 & 17 \\ 
OGLE0915 & -0.47 & 0.09 & 0.07 & 101 & -0.46 & 0.07 & 0.08 & 14 \\ 
OGLE0936 & -0.49 & 0.11 & 0.04 & 93 & -0.52 & 0.15 & 0.03 & 17 \\ 
OGLE0949 & -0.43 & 0.09 & 0.07 & 83 & -0.43 & 0.08 & 0.06 & 12 \\ 
OGLE0966 & -0.44 & 0.12 & 0.05 & 73 & -0.45 & 0.07 & 0.02 & 9 \\ 
OGLE0969 & -0.38 & 0.11 & 0.04 & 94 & -0.39 & 0.07 & 0.04 & 15 \\ 
OGLE0970 & -0.32 & 0.10 & 0.06 & 82 & -0.34 & 0.10 & 0.04 & 13 \\ 
OGLE0975 & -0.40 & 0.11 & 0.09 & 75 & -0.43 & 0.14 & 0.06 & 14 \\ 
OGLE0978 & -0.43 & 0.10 & 0.04 & 80 & -0.43 & 0.07 & 0.05 & 12 \\ 
OGLE0986 & -0.40 & 0.10 & 0.09 & 69 & -0.45 & 0.16 & 0.08 & 8 \\ 
OGLE0992 & -0.41 & 0.08 & 0.05 & 64 & -0.39 & 0.18 & 0.07 & 7 \\ 
OGLE1001 & -0.31 & 0.12 & 0.05 & 92 & -0.34 & 0.10 & 0.02 & 12 \\ 
OGLE1031 & -0.41 & 0.10 & 0.05 & 69 & -0.43 & 0.09 & 0.02 & 13 \\ 
OGLE1058 & -0.46 & 0.13 & 0.15 & 66 & -0.45 & 0.21 & 0.15 & 14 \\ 
OGLE1080 & -0.49 & 0.16 & 0.08 & 73 & -0.48 & 0.09 & 0.06 & 8 \\ 
OGLE1109 & -0.48 & 0.11 & 0.07 & 90 & -0.50 & 0.07 & 0.06 & 13 \\ 
OGLE1112 & -0.34 & 0.14 & 0.10 & 83 & -0.37 & 0.09 & 0.07 & 12 \\ 
OGLE1313 & -0.79 & 0.09 & 0.13 & 82 & -0.82 & 0.07 & 0.10 & 12 \\ 
OGLE1374 & -0.63 & 0.10 & 0.08 & 75 & -0.67 & 0.09 & 0.08 & 10 \\ 
OGLE1389 & -0.43 & 0.10 & 0.05 & 97 & -0.44 & 0.12 & 0.05 & 15 \\ 
OGLE1411 & -0.49 & 0.11 & 0.07 & 90 & -0.54 & 0.08 & 0.04 & 13 \\ 
OGLE1417 & -0.41 & 0.07 & 0.05 & 70 & -0.44 & 0.05 & 0.03 & 12 \\ 
OGLE1424 & -0.45 & 0.09 & 0.07 & 90 & -0.46 & 0.13 & 0.05 & 14 \\ 
OGLE1431 & -0.33 & 0.08 & 0.06 & 81 & -0.33 & 0.11 & 0.05 & 13 \\ 
OGLE1463 & -0.35 & 0.12 & 0.08 & 86 & -0.41 & 0.11 & 0.03 & 15 \\ 
OGLE1466 & -0.37 & 0.08 & 0.07 & 77 & -0.41 & 0.09 & 0.05 & 13 \\ 
OGLE1490 & -0.53 & 0.11 & 0.07 & 108 & -0.56 & 0.15 & 0.06 & 17 \\ 
OGLE1526 & -0.34 & 0.12 & 0.08 & 89 & -0.37 & 0.11 & 0.05 & 13 \\ 
OGLE1539 & -0.41 & 0.14 & 0.05 & 81 & -0.41 & 0.06 & 0.04 & 14 \\ 
OGLE1578 & -0.30 & 0.11 & 0.06 & 78 & -0.29 & 0.12 & 0.07 & 11 \\ 
OGLE1587 & -0.29 & 0.13 & 0.05 & 68 & -0.32 & 0.03 & 0.02 & 7 \\ 
OGLE1616 & -0.27 & 0.11 & 0.04 & 96 & -0.27 & 0.14 & 0.04 & 16 \\ 
OGLE1637 & -0.35 & 0.12 & 0.08 & 69 & -0.35 & 0.04 & 0.06 & 6 \\ 
OGLE1641 & -0.34 & 0.10 & 0.10 & 89 & -0.37 & 0.15 & 0.07 & 15 \\ 
OGLE1647 & -0.33 & 0.11 & 0.07 & 89 & -0.33 & 0.10 & 0.06 & 14 \\ 
OGLE1677 & -0.31 & 0.12 & 0.08 & 85 & -0.31 & 0.14 & 0.08 & 14 \\ 
OGLE1862 & -0.36 & 0.09 & 0.04 & 85 & -0.34 & 0.09 & 0.06 & 15 \\ 
OGLE1939 & -0.37 & 0.07 & 0.13 & 58 & -0.40 & 0.14 & 0.12 & 13 \\ 
OGLE1941 & -0.22 & 0.09 & 0.06 & 87 & -0.22 & 0.08 & 0.05 & 13 \\ 
OGLE1994 & -0.29 & 0.10 & 0.08 & 93 & -0.32 & 0.14 & 0.06 & 18 \\ 
OGLE2012 & -0.38 & 0.11 & 0.05 & 98 & -0.37 & 0.09 & 0.05 & 14 \\ 
OGLE2019 & -0.13 & 0.15 & 0.06 & 52 & -0.13 & 0.11 & 0.05 & 7 \\ 
OGLE2043 & -0.41 & 0.08 & 0.06 & 86 & -0.41 & 0.09 & 0.05 & 13 \\ 
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abus/Fe_abundances10.tex <==
OGLE0434 & -0.40 & 0.12 & 0.07 & 101 & -0.43 & 0.13 & 0.04 & 15 \\ 
OGLE0501 & -0.42 & 0.09 & 0.05 & 84 & -0.43 & 0.06 & 0.03 & 12 \\ 
OGLE0510 & -0.38 & 0.11 & 0.03 & 82 & -0.39 & 0.14 & 0.03 & 9 \\ 
OGLE0512 & -0.48 & 0.13 & 0.06 & 91 & -0.41 & 0.11 & 0.01 & 14 \\ 
OGLE0528 & -0.41 & 0.12 & 0.04 & 91 & -0.43 & 0.07 & 0.02 & 15 \\ 
OGLE0545 & -0.37 & 0.09 & 0.06 & 78 & -0.40 & 0.04 & 0.05 & 10 \\ 
OGLE0590 & -0.41 & 0.10 & 0.23 & 83 & -0.38 & 0.13 & 0.08 & 15 \\ 
OGLE0594 & -0.49 & 0.14 & 0.12 & 71 & -0.50 & 0.02 & 0.10 & 6 \\ 
OGLE0648 & -0.45 & 0.09 & 0.06 & 98 & -0.47 & 0.09 & 0.04 & 17 \\ 
OGLE0683 & -0.38 & 0.11 & 0.07 & 90 & -0.40 & 0.14 & 0.05 & 16 \\ 
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abus/O_abundances.tex <==
OGLE0434 & -0.36 & 0.10 & 2 \\ 
OGLE0501 & -0.21 & 0.10 & 2 \\ 
OGLE0510 & -0.30 & 0.06 & 1 \\ 
OGLE0512 & -0.35 & 0.06 & 2 \\ 
OGLE0528 & -0.29 & 0.07 & 2 \\ 
OGLE0545 & -0.22 & 0.10 & 1 \\ 
OGLE0590 & ---- & --- & --- \\ 
OGLE0594 & -0.12 & 0.21 & 1 \\ 
OGLE0648 & -0.32 & 0.11 & 1 \\ 
OGLE0683 & -0.28 & 0.12 & 1 \\ 
OGLE0712 & -0.24 & 0.10 & 2 \\ 
OGLE0716 & -0.24 & 0.09 & 2 \\ 
OGLE0727 & ---- & --- & --- \\ 
OGLE0757 & ---- & --- & --- \\ 
OGLE0770 & -0.47 & 0.10 & 1 \\ 
OGLE0787 & ---- & --- & --- \\ 
OGLE0798 & ---- & --- & --- \\ 
OGLE0800 & ---- & --- & --- \\ 
OGLE0812 & -0.05 & 0.12 & 1 \\ 
OGLE0819 & -0.10 & 0.07 & 1 \\ 
OGLE0821 & -0.43 & 0.08 & 1 \\ 
OGLE0831 & -0.28 & 0.10 & 2 \\ 
OGLE0844 & ---- & --- & --- \\ 
OGLE0847 & -0.29 & 0.09 & 2 \\ 
OGLE0848 & ---- & --- & --- \\ 
OGLE0888 & ---- & --- & --- \\ 
OGLE0915 & -0.36 & 0.13 & 2 \\ 
OGLE0936 & ---- & --- & --- \\ 
OGLE0949 & ---- & --- & --- \\ 
OGLE0966 & -0.42 & 0.05 & 1 \\ 
OGLE0969 & -0.30 & 0.08 & 2 \\ 
OGLE0970 & -0.20 & 0.08 & 1 \\ 
OGLE0975 & ---- & --- & --- \\ 
OGLE0978 & -0.32 & 0.09 & 1 \\ 
OGLE0986 & ---- & --- & --- \\ 
OGLE0992 & -0.32 & 0.11 & 1 \\ 
OGLE1001 & -0.16 & 0.07 & 2 \\ 
OGLE1031 & -0.38 & 0.07 & 1 \\ 
OGLE1058 & 0.04 & 0.27 & 2 \\ 
OGLE1080 & ---- & --- & --- \\ 
OGLE1109 & -0.42 & 0.12 & 1 \\ 
OGLE1112 & 0.19 & 0.13 & 1 \\ 
OGLE1313 & -0.03 & 0.23 & 2 \\ 
OGLE1374 & -0.09 & 0.16 & 1 \\ 
OGLE1389 & -0.40 & 0.10 & 1 \\ 
OGLE1411 & -0.52 & 0.10 & 1 \\ 
OGLE1417 & ---- & --- & --- \\ 
OGLE1424 & ---- & --- & --- \\ 
OGLE1431 & -0.00 & 0.10 & 1 \\ 
OGLE1463 & ---- & --- & --- \\ 
OGLE1466 & -0.24 & 0.09 & 1 \\ 
OGLE1490 & -0.61 & 0.12 & 1 \\ 
OGLE1526 & ---- & --- & --- \\ 
OGLE1539 & -0.08 & 0.09 & 1 \\ 
OGLE1578 & ---- & --- & --- \\ 
OGLE1587 & ---- & --- & --- \\ 
OGLE1616 & -0.22 & 0.08 & 1 \\ 
OGLE1637 & -0.40 & 0.11 & 1 \\ 
OGLE1641 & ---- & --- & --- \\ 
OGLE1647 & ---- & --- & --- \\ 
OGLE1677 & 0.06 & 0.14 & 1 \\ 
OGLE1862 & -0.31 & 0.11 & 1 \\ 
OGLE1939 & ---- & --- & --- \\ 
OGLE1941 & 0.00 & 0.10 & 2 \\ 
OGLE1994 & ---- & --- & --- \\ 
OGLE2012 & -0.31 & 0.10 & 1 \\ 
OGLE2019 & ---- & --- & --- \\ 
OGLE2043 & ---- & --- & --- \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abus/O_abundances10.tex <==
OGLE0434 & -0.36 & 0.10 & 2 \\ 
    OGLE0501 & -0.21 & 0.10 & 2 \\ 
OGLE0510 & -0.30 & 0.06 & 1 \\ 
OGLE0512 & -0.35 & 0.06 & 2 \\ 
OGLE0528 & -0.29 & 0.07 & 2 \\ 
OGLE0545 & -0.22 & 0.10 & 1 \\ 
OGLE0590 & ---- & --- & --- \\ 
OGLE0594 & -0.12 & 0.21 & 1 \\ 
OGLE0648 & -0.32 & 0.11 & 1 \\ 
OGLE0683 & -0.28 & 0.12 & 1 \\ 
\ldots & \ldots & \ldots & \ldots \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abus/parameters.tex <==
OGLE0434 & 5660 & 100 & 0.30 & 0.13 & 2.90 & 0.10 & 0.2577 \\ 
OGLE0501 & 5130 & 77 & 0.30 & 0.05 & 3.10 & 0.09 & 0.4385 \\ 
OGLE0510 & 5530 & 64 & 0.10 & 0.15 & 3.70 & 0.14 & 0.1274 \\ 
OGLE0512 & 5200 & 79 & 0.00 & 0.09 & 3.50 & 0.15 & 0.1892 \\ 
OGLE0528 & 5200 & 64 & 0.10 & 0.08 & 3.50 & 0.19 & 0.3005 \\ 
OGLE0545 & 5420 & 85 & 0.80 & 0.05 & 3.90 & 0.15 & 0.8352 \\ 
OGLE0590 & 5880 & 322 & 0.00 & 0.10 & 3.60 & 0.09 & 0.1314 \\ 
OGLE0594 & 5520 & 194 & 0.90 & 0.05 & 3.60 & 0.23 & 0.6911 \\ 
OGLE0648 & 5300 & 90 & 0.50 & 0.07 & 2.90 & 0.08 & 0.2372 \\ 
OGLE0683 & 5560 & 105 & 0.40 & 0.12 & 3.00 & 0.09 & 0.1281 \\ 
OGLE0712 & 5630 & 77 & 0.50 & 0.10 & 2.90 & 0.09 & 0.3109 \\ 
OGLE0716 & 5130 & 71 & 0.50 & 0.07 & 2.60 & 0.08 & 0.3489 \\ 
OGLE0727 & 5490 & 240 & 0.60 & 0.08 & 4.00 & 0.13 & 0.7902 \\ 
OGLE0757 & 5390 & 100 & 0.90 & 0.08 & 3.70 & 0.13 & 0.5455 \\ 
OGLE0770 & 5130 & 73 & 0.40 & 0.04 & 2.90 & 0.07 & 0.4226 \\ 
OGLE0787 & 4980 & 69 & 0.50 & 0.09 & 4.00 & 0.43 & 0.6923 \\ 
OGLE0798 & 5220 & 83 & 0.70 & 0.07 & 4.00 & 0.18 & 0.5864 \\ 
OGLE0800 & 5830 & 138 & 0.50 & 0.10 & 3.00 & 0.08 & 0.9702 \\ 
OGLE0812 & 6100 & 118 & 0.50 & 0.12 & 2.70 & 0.11 & 0.0206 \\ 
OGLE0819 & 5060 & 55 & 0.70 & 0.06 & 3.40 & 0.16 & 0.4384 \\ 
OGLE0821 & 5160 & 89 & 0.00 & 0.07 & 3.30 & 0.11 & 0.2397 \\ 
OGLE0831 & 5190 & 84 & 0.70 & 0.07 & 3.50 & 0.14 & 0.4606 \\ 
OGLE0844 & 5920 & 141 & 0.40 & 0.13 & 3.40 & 0.14 & 0.1058 \\ 
OGLE0847 & 4930 & 81 & 0.20 & 0.06 & 3.20 & 0.11 & 0.5323 \\ 
OGLE0848 & 5430 & 141 & 0.80 & 0.06 & 3.90 & 0.13 & 0.8285 \\ 
OGLE0888 & 5590 & 87 & 0.60 & 0.10 & 2.80 & 0.07 & 0.9559 \\ 
OGLE0915 & 5430 & 98 & 1.00 & 0.07 & 3.10 & 0.08 & 0.4092 \\ 
OGLE0936 & 5980 & 79 & 0.60 & 0.10 & 3.00 & 0.13 & 0.9814 \\ 
OGLE0949 & 5520 & 95 & 0.80 & 0.06 & 3.90 & 0.17 & 0.8493 \\ 
OGLE0966 & 4900 & 62 & 0.00 & 0.07 & 4.00 & 0.23 & 0.6380 \\ 
OGLE0969 & 5130 & 62 & 0.70 & 0.06 & 3.20 & 0.18 & 0.3468 \\ 
OGLE0970 & 5550 & 80 & 0.50 & 0.08 & 3.40 & 0.12 & 0.1037 \\ 
OGLE0975 & 5690 & 129 & 0.60 & 0.10 & 3.30 & 0.14 & 0.1243 \\ 
OGLE0978 & 5250 & 73 & 0.60 & 0.06 & 3.70 & 0.16 & 0.2940 \\ 
OGLE0986 & 5430 & 132 & 0.10 & 0.15 & 4.00 & 0.16 & 0.9396 \\ 
OGLE0992 & 5370 & 75 & 0.20 & 0.17 & 4.00 & 0.16 & 0.5211 \\ 
OGLE1001 & 5030 & 67 & 0.50 & 0.08 & 3.40 & 0.12 & 0.4434 \\ 
OGLE1031 & 4830 & 59 & 0.40 & 0.06 & 3.70 & 0.13 & 0.5862 \\ 
OGLE1058 & 6060 & 262 & 0.70 & 0.15 & 3.20 & 0.13 & 0.9624 \\ 
OGLE1080 & 5030 & 100 & 0.50 & 0.07 & 4.00 & 0.39 & 0.7434 \\ 
OGLE1109 & 5360 & 100 & 0.80 & 0.06 & 3.60 & 0.14 & 0.6667 \\ 
OGLE1112 & 5620 & 143 & 0.70 & 0.10 & 3.40 & 0.16 & 0.3076 \\ 
OGLE1313 & 6000 & 232 & 0.90 & 0.08 & 3.30 & 0.11 & 0.9292 \\ 
OGLE1374 & 5360 & 143 & 0.60 & 0.09 & 3.70 & 0.16 & 0.3794 \\ 
OGLE1389 & 5530 & 86 & 0.70 & 0.11 & 2.80 & 0.07 & 0.2840 \\ 
OGLE1411 & 5360 & 88 & 0.70 & 0.06 & 3.90 & 0.19 & 0.7261 \\ 
OGLE1417 & 5350 & 74 & 0.70 & 0.05 & 3.90 & 0.12 & 0.4316 \\ 
OGLE1424 & 5730 & 115 & 0.80 & 0.09 & 3.20 & 0.10 & 0.0006 \\ 
OGLE1431 & 5560 & 87 & 0.90 & 0.07 & 3.70 & 0.11 & 0.7531 \\ 
OGLE1463 & 5830 & 119 & 0.50 & 0.10 & 3.00 & 0.09 & 0.1260 \\ 
OGLE1466 & 5720 & 108 & 0.90 & 0.07 & 3.50 & 0.10 & 0.9098 \\ 
OGLE1490 & 5760 & 123 & 0.70 & 0.26 & 2.60 & 0.07 & 0.2465 \\ 
OGLE1526 & 5400 & 114 & 0.90 & 0.09 & 3.90 & 0.14 & 0.7563 \\ 
OGLE1539 & 4970 & 67 & 0.70 & 0.05 & 3.70 & 0.20 & 0.5316 \\ 
OGLE1578 & 5600 & 99 & 1.00 & 0.10 & 3.90 & 0.17 & 0.8202 \\ 
OGLE1587 & 5090 & 63 & 0.60 & 0.05 & 4.00 & 0.31 & 0.6855 \\ 
OGLE1616 & 5420 & 70 & 0.40 & 0.14 & 2.80 & 0.08 & 0.3429 \\ 
OGLE1637 & 5160 & 98 & 0.30 & 0.06 & 4.00 & 0.30 & 0.7816 \\ 
OGLE1641 & 6150 & 152 & 0.40 & 0.12 & 3.20 & 0.12 & 0.0697 \\ 
OGLE1647 & 5790 & 95 & 1.00 & 0.08 & 3.60 & 0.11 & 0.8869 \\ 
OGLE1677 & 6050 & 138 & 0.20 & 0.11 & 3.00 & 0.10 & 0.0333 \\ 
OGLE1862 & 5170 & 65 & 0.60 & 0.07 & 3.10 & 0.10 & 0.2332 \\ 
OGLE1939 & 5550 & 210 & 0.90 & 0.11 & 3.10 & 0.07 & 0.8346 \\ 
OGLE1941 & 5420 & 89 & 1.20 & 0.08 & 3.40 & 0.10 & 0.4380 \\ 
OGLE1994 & 6420 & 137 & 0.90 & 0.11 & 2.80 & 0.08 & 0.9900 \\ 
OGLE2012 & 5660 & 91 & 0.80 & 0.08 & 2.80 & 0.08 & 0.1205 \\ 
OGLE2019 & 5030 & 66 & 0.70 & 0.15 & 4.00 & 0.49 & 0.7111 \\ 
OGLE2043 & 5460 & 99 & 0.80 & 0.07 & 3.10 & 0.08 & 0.3209 \\ 
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abus/parameters10.tex <==
OGLE0434 & 5660 & 100 & 0.30 & 0.13 & 2.90 & 0.10 & 0.2577 \\ 
OGLE0501 & 5130 & 77 & 0.30 & 0.05 & 3.10 & 0.09 & 0.4385 \\ 
OGLE0510 & 5530 & 64 & 0.10 & 0.15 & 3.70 & 0.14 & 0.1274 \\ 
OGLE0512 & 5200 & 79 & 0.00 & 0.09 & 3.50 & 0.15 & 0.1892 \\ 
OGLE0528 & 5200 & 64 & 0.10 & 0.08 & 3.50 & 0.19 & 0.3005 \\ 
OGLE0545 & 5420 & 85 & 0.80 & 0.05 & 3.90 & 0.15 & 0.8352 \\ 
OGLE0590 & 5880 & 322 & 0.00 & 0.10 & 3.60 & 0.09 & 0.1314 \\ 
OGLE0594 & 5520 & 194 & 0.90 & 0.05 & 3.60 & 0.23 & 0.6911 \\ 
OGLE0648 & 5300 & 90 & 0.50 & 0.07 & 2.90 & 0.08 & 0.2372 \\ 
OGLE0683 & 5560 & 105 & 0.40 & 0.12 & 3.00 & 0.09 & 0.1281 \\ 
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abusR08/R08_Fe_abundances.tex <==
OGLE107 & -0.43 & 0.09 & 0.03 & 101 & -0.46 & 0.09 & 0.04 & 17 \\ 
OGLE461 & -0.30 & 0.15 & 0.09 & 65 & -0.30 & 0.08 & 0.10 & 9 \\ 
OGLE655 & -0.41 & 0.11 & 0.06 & 94 & -0.43 & 0.14 & 0.05 & 17 \\ 
OGLE945 & -0.53 & 0.09 & 0.04 & 83 & -0.47 & 0.09 & 0.00 & 14 \\ 
OGLE1100 & -0.33 & 0.12 & 0.07 & 79 & -0.35 & 0.19 & 0.04 & 18 \\ 
OGLE1128 & -0.51 & 0.12 & 0.04 & 82 & -0.51 & 0.10 & 0.05 & 13 \\ 
OGLE1290 & -0.37 & 0.13 & 0.05 & 59 & -0.36 & 0.07 & 0.04 & 7 \\ 
OGLE1327 & -0.50 & 0.15 & 0.08 & 81 & -0.52 & 0.10 & 0.06 & 13 \\ 
OGLE2337 & -0.36 & 0.09 & 0.04 & 87 & -0.36 & 0.11 & 0.04 & 15 \\ 
OGLE2832 & -0.28 & 0.15 & 0.12 & 63 & -0.30 & 0.10 & 0.12 & 9 \\ 
OGLE2949 & -0.44 & 0.11 & 0.03 & 88 & -0.45 & 0.10 & 0.05 & 15 \\ 
OGLE3158 & -0.45 & 0.09 & 0.06 & 78 & -0.44 & 0.13 & 0.06 & 14 \\ 
OGLE3320 & -0.40 & 0.12 & 0.05 & 75 & -0.41 & 0.13 & 0.06 & 9 \\ 
OGLE4033 & -0.78 & 0.09 & 0.04 & 97 & -0.76 & 0.09 & 0.04 & 16 \\ 
OGLE4061 & -0.44 & 0.09 & 0.03 & 89 & -0.46 & 0.09 & 0.02 & 15 \\ 
OGLE4208 & -0.55 & 0.09 & 0.03 & 80 & -0.56 & 0.09 & 0.02 & 14 \\ 
OGLE4357 & -0.47 & 0.08 & 0.04 & 89 & -0.46 & 0.07 & 0.04 & 15 \\ 
OGLE4451 & -0.51 & 0.10 & 0.07 & 90 & -0.51 & 0.10 & 0.09 & 16 \\ 
OGLE4544 & -0.44 & 0.07 & 0.03 & 77 & -0.44 & 0.08 & 0.02 & 12 \\ 
OGLE4628 & -0.53 & 0.10 & 0.07 & 67 & -0.32 & 0.16 & -0.02 & 9 \\ 
OGLE4689 & -0.40 & 0.12 & 0.08 & 68 & -0.38 & 0.06 & 0.02 & 7 \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abusR08/R08_Fe_abundances10.tex <==
OGLE107 & -0.43 & 0.09 & 0.03 & 101 & -0.46 & 0.09 & 0.04 & 17 \\ 
OGLE461 & -0.30 & 0.15 & 0.09 & 65 & -0.30 & 0.08 & 0.10 & 9 \\ 
OGLE655 & -0.41 & 0.11 & 0.06 & 94 & -0.43 & 0.14 & 0.05 & 17 \\ 
OGLE945 & -0.53 & 0.09 & 0.04 & 83 & -0.47 & 0.09 & 0.00 & 14 \\ 
OGLE1100 & -0.33 & 0.12 & 0.07 & 79 & -0.35 & 0.19 & 0.04 & 18 \\ 
OGLE1128 & -0.51 & 0.12 & 0.04 & 82 & -0.51 & 0.10 & 0.05 & 13 \\ 
OGLE1290 & -0.37 & 0.13 & 0.05 & 59 & -0.36 & 0.07 & 0.04 & 7 \\ 
OGLE1327 & -0.50 & 0.15 & 0.08 & 81 & -0.52 & 0.10 & 0.06 & 13 \\ 
OGLE2337 & -0.36 & 0.09 & 0.04 & 87 & -0.36 & 0.11 & 0.04 & 15 \\ 
OGLE2832 & -0.28 & 0.15 & 0.12 & 63 & -0.30 & 0.10 & 0.12 & 9 \\ 
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abusR08/R08_O_abundances.tex <==
OGLE107 & -0.33 & 0.06 & 2 \\ 
OGLE461 & 0.03 & 0.18 & 2 \\ 
OGLE655 & -0.28 & 0.10 & 1 \\ 
OGLE945 & -0.38 & 0.03 & 2 \\ 
OGLE1100 & 0.02 & 0.10 & 2 \\ 
OGLE1128 & -0.33 & 0.09 & 1 \\ 
OGLE1290 & -0.29 & 0.07 & 1 \\ 
OGLE1327 & -0.17 & 0.12 & 1 \\ 
OGLE2337 & -0.33 & 0.07 & 1 \\ 
OGLE2832 & ---- & --- & --- \\ 
OGLE2949 & -0.37 & 0.08 & 1 \\ 
OGLE3158 & ---- & --- & --- \\ 
OGLE3320 & 0.43 & 0.10 & 1 \\ 
OGLE4033 & ---- & --- & --- \\ 
OGLE4061 & -0.44 & 0.07 & 1 \\ 
OGLE4208 & -0.37 & 0.04 & 1 \\ 
OGLE4357 & -0.40 & 0.07 & 1 \\ 
OGLE4451 & -0.29 & 0.12 & 1 \\ 
OGLE4544 & -0.43 & 0.05 & 1 \\ 
OGLE4628 & -0.34 & 0.02 & 1 \\ 
OGLE4689 & -0.29 & 0.07 & 1 \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abusR08/R08_O_abundances10.tex <==
OGLE107 & -0.33 & 0.06 & 2 \\ 
OGLE461 & 0.03 & 0.18 & 2 \\ 
OGLE655 & -0.28 & 0.10 & 1 \\ 
OGLE945 & -0.38 & 0.03 & 2 \\ 
OGLE1100 & 0.02 & 0.10 & 2 \\ 
OGLE1128 & -0.33 & 0.09 & 1 \\ 
OGLE1290 & -0.29 & 0.07 & 1 \\ 
OGLE1327 & -0.17 & 0.12 & 1 \\ 
OGLE2337 & -0.33 & 0.07 & 1 \\ 
OGLE2832 & ---- & --- & --- \\ 
\ldots & \ldots & \ldots & \ldots \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abusR08/R08_parameters.tex <==
OGLE107 & 5390 & 42 & 0.80 & 0.07 & 2.80 & 0.06 & 0.860 \\ 
OGLE461 & 4890 & 109 & 0.70 & 0.08 & 4.00 & 0.51 & 0.682 \\ 
OGLE655 & 5590 & 86 & 0.50 & 0.11 & 3.20 & 0.11 & 0.144 \\ 
OGLE945 & 4960 & 40 & 0.00 & 0.09 & 3.60 & 0.12 & 0.605 \\ 
OGLE1100 & 6200 & 122 & 0.70 & 0.16 & 3.10 & 0.17 & 0.201 \\ 
OGLE1128 & 5370 & 65 & 0.80 & 0.09 & 3.70 & 0.19 & 0.861 \\ 
OGLE1290 & 4870 & 64 & 0.10 & 0.08 & 4.00 & 1.04 & 0.136 \\ 
OGLE1327 & 5660 & 122 & 0.70 & 0.09 & 3.20 & 0.16 & 0.037 \\ 
OGLE2337 & 5590 & 56 & 0.40 & 0.09 & 3.20 & 0.12 & 0.130 \\ 
OGLE2832 & 5060 & 164 & 0.80 & 0.10 & 4.00 & 0.63 & 0.710 \\ 
OGLE2949 & 5230 & 51 & 0.20 & 0.11 & 3.20 & 0.12 & 0.917 \\ 
OGLE3158 & 5630 & 108 & 0.20 & 0.10 & 3.40 & 0.14 & 0.144 \\ 
OGLE3320 & 5880 & 87 & 1.40 & 0.15 & 3.70 & 0.20 & 0.024 \\ 
OGLE4033 & 5500 & 72 & 0.60 & 0.09 & 2.60 & 0.08 & 0.237 \\ 
OGLE4061 & 5230 & 49 & 0.20 & 0.08 & 3.00 & 0.08 & 0.119 \\ 
OGLE4208 & 5290 & 38 & 0.80 & 0.08 & 3.60 & 0.12 & 0.411 \\ 
OGLE4357 & 5290 & 47 & 0.20 & 0.07 & 3.40 & 0.12 & 0.059 \\ 
OGLE4451 & 5530 & 92 & 0.70 & 0.10 & 3.00 & 0.09 & 0.055 \\ 
OGLE4544 & 5330 & 36 & 0.70 & 0.08 & 3.20 & 0.11 & 0.342 \\ 
OGLE4628 & 4900 & 65 & 0.00 & 0.13 & 4.00 & 0.23 & 0.321 \\ 
OGLE4689 & 4840 & 94 & 0.00 & 0.07 & 4.00 & 0.23 & 0.880 \\ 


==> SH0ES LMC spectroscopy(1)/Tables/params_abusR08/R08_parameters10.tex <==
OGLE107 & 5390 & 42 & 0.80 & 0.07 & 2.80 & 0.06 & 0.860 \\ 
OGLE461 & 4890 & 109 & 0.70 & 0.08 & 4.00 & 0.51 & 0.682 \\ 
OGLE655 & 5590 & 86 & 0.50 & 0.11 & 3.20 & 0.11 & 0.144 \\ 
OGLE945 & 4960 & 40 & 0.00 & 0.09 & 3.60 & 0.12 & 0.605 \\ 
OGLE1100 & 6200 & 122 & 0.70 & 0.16 & 3.10 & 0.17 & 0.201 \\ 
OGLE1128 & 5370 & 65 & 0.80 & 0.09 & 3.70 & 0.19 & 0.861 \\ 
OGLE1290 & 4870 & 64 & 0.10 & 0.08 & 4.00 & 1.04 & 0.136 \\ 
OGLE1327 & 5660 & 122 & 0.70 & 0.09 & 3.20 & 0.16 & 0.037 \\ 
OGLE2337 & 5590 & 56 & 0.40 & 0.09 & 3.20 & 0.12 & 0.130 \\ 
OGLE2832 & 5060 & 164 & 0.80 & 0.10 & 4.00 & 0.63 & 0.710 \\ 
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\ 


==> Tables/linelist/linelist.tex <==
4892.86 & FeI & -0.876 & 4.22 \\
4893.81 & FeII & -4.157 & 2.83 \\
4917.23 & FeI & -1.160 & 4.19 \\
4923.92 & FeII & -1.559 & 2.89 \\
4924.77 & FeI & -2.114 & 2.28 \\
4932.08 & FeI & -1.483 & 4.65 \\
4950.10 & FeI & -1.500 & 3.42 \\
4973.10 & FeI & -0.690 & 3.96 \\
4993.35 & FeII & -3.684 & 2.81 \\
4994.13 & FeI & -3.080 & 0.92 \\
5029.62 & FeI & -2.000 & 3.42 \\
5044.21 & FeI & -2.017 & 2.85 \\
5049.82 & FeI & -1.355 & 2.28 \\
5054.64 & FeI & -1.921 & 3.64 \\
5056.84 & FeI & -1.940 & 4.26 \\
5067.15 & FeI & -0.484 & 4.22 \\
5072.67 & FeI & -0.834 & 4.22 \\
5083.34 & FeI & -2.958 & 0.96 \\
5090.77 & FeI & -0.440 & 4.26 \\
5100.65 & FeII & -4.222 & 2.81 \\
5126.19 & FeI & -1.060 & 4.26 \\
5132.67 & FeII & -6.427 & 6.73 \\
5133.69 & FeI & 0.360 & 4.18 \\
5171.60 & FeI & -1.793 & 1.49 \\
5197.58 & FeII & -3.575 & 12.89 \\
5198.71 & FeI & -2.135 & 2.22 \\
5215.18 & FeI & -0.860 & 3.27 \\
5216.27 & FeI & -2.150 & 1.61 \\
5217.39 & FeI & -1.070 & 3.21 \\
5234.62 & FeII & -2.138 & 3.22 \\
5242.49 & FeI & -0.967 & 3.63 \\
5243.78 & FeI & -1.120 & 4.26 \\
5256.93 & FeII & -4.327 & 2.89 \\
5257.65 & FeI & -2.753 & 3.57 \\
5281.79 & FeI & -0.834 & 3.04 \\
5288.53 & FeI & -1.490 & 3.69 \\
5307.36 & FeI & -2.987 & 1.61 \\
5324.18 & FeI & -0.110 & 3.21 \\
5325.55 & FeII & -3.185 & 3.22 \\
5326.14 & FeI & -2.071 & 3.57 \\
5339.93 & FeI & -0.630 & 3.27 \\
5362.86 & FeII & -2.616 & 3.20 \\
5364.87 & FeI & 0.228 & 4.45 \\
5365.40 & FeI & -1.020 & 3.57 \\
5367.47 & FeI & 0.443 & 4.42 \\
5373.71 & FeI & -0.710 & 4.47 \\
5379.57 & FeI & -1.514 & 3.69 \\
5383.37 & FeI & 0.645 & 4.31 \\
5389.49 & FeI & -7.973 & 5.33 \\
5391.46 & FeI & -0.777 & 4.15 \\
5393.17 & FeI & -0.720 & 3.24 \\
5398.28 & FeI & -0.710 & 4.45 \\
5405.77 & FeI & -1.844 & 0.99 \\
5410.91 & FeI & 0.398 & 4.47 \\
5414.07 & FeII & -3.644 & 3.22 \\
5415.20 & FeI & 0.642 & 4.39 \\
5417.04 & FeI & -1.660 & 4.42 \\
5424.07 & FeI & 0.778 & 4.32 \\
5425.25 & FeII & -3.352 & 3.20 \\
5434.52 & FeI & -2.122 & 1.01 \\
5445.04 & FeI & 0.211 & 4.39 \\
5452.09 & FeI & -2.812 & 3.64 \\
5464.28 & FeI & -1.400 & 4.14 \\
5466.40 & FeI & -0.285 & 4.37 \\
5497.52 & FeI & -2.849 & 1.01 \\
5501.47 & FeI & -3.047 & 0.96 \\
5506.78 & FeI & -2.797 & 0.99 \\
5522.45 & FeI & -1.520 & 4.21 \\
5531.98 & FeI & -1.600 & 4.91 \\
5534.84 & FeII & -2.865 & 3.25 \\
5543.15 & FeI & -4.651 & 3.69 \\
5554.89 & FeI & -0.270 & 4.55 \\
5560.21 & FeI & -1.160 & 4.43 \\
5561.24 & FeI & -1.204 & 4.61 \\
5562.70 & FeI & -0.642 & 4.43 \\
5565.70 & FeI & -0.214 & 4.61 \\
5572.84 & FeI & -0.280 & 3.40 \\
5576.09 & FeI & -0.940 & 3.43 \\
5584.76 & FeI & -2.270 & 3.57 \\
5586.77 & FeI & -2.903 & 4.26 \\
5627.49 & FeII & -4.062 & 3.39 \\
5633.95 & FeI & -0.320 & 4.99 \\
5635.85 & FeI & -9.120 & 5.37 \\
5638.26 & FeI & -0.720 & 4.22 \\
5641.43 & FeI & -1.150 & 4.26 \\
5653.86 & FeI & -1.610 & 4.39 \\
5658.82 & FeI & -0.760 & 3.40 \\
5661.34 & FeI & -1.756 & 4.28 \\
5679.02 & FeI & -0.900 & 4.65 \\
5686.53 & FeI & -0.446 & 4.55 \\
5691.50 & FeI & -1.490 & 4.30 \\
5707.05 & FeI & -2.350 & 3.64 \\
5717.83 & FeI & -0.960 & 4.28 \\
5720.89 & FeI & -1.632 & 4.55 \\
5731.76 & FeI & -1.270 & 4.26 \\
5834.02 & FeI & -0.979 & 4.91 \\
5835.10 & FeI & -2.040 & 4.26 \\
5838.37 & FeI & -2.290 & 3.94 \\
5848.13 & FeI & -1.057 & 4.61 \\
5849.68 & FeI & -2.633 & 3.69 \\
5852.21 & FeI & -5.954 & 5.62 \\
5853.15 & FeI & -4.254 & 1.49 \\
5855.07 & FeI & -1.478 & 4.61 \\
5856.09 & FeI & -1.328 & 4.29 \\
5858.78 & FeI & -2.349 & 4.22 \\
5859.59 & FeI & -0.418 & 4.55 \\
5861.11 & FeI & -2.268 & 4.28 \\
5862.36 & FeI & -0.125 & 4.55 \\
5873.21 & FeI & -2.109 & 4.26 \\
5877.79 & FeI & -2.233 & 4.18 \\
5883.82 & FeI & -1.310 & 3.96 \\
5885.05 & FeI & -1.479 & 4.99 \\
5902.47 & FeI & -1.313 & 4.59 \\
5902.55 & FeI & -2.695 & 5.87 \\
5905.67 & FeI & -0.770 & 4.65 \\
5916.25 & FeI & -2.994 & 2.45 \\
5921.26 & FeI & -0.685 & 4.65 \\
5927.79 & FeI & -1.070 & 4.65 \\
5929.68 & FeI & -1.380 & 4.55 \\
5930.18 & FeI & -0.057 & 4.65 \\
5934.65 & FeI & -1.120 & 3.93 \\
5940.99 & FeI & -1.638 & 4.18 \\
5943.58 & FeI & -4.192 & 2.20 \\
5956.69 & FeI & -4.608 & 0.86 \\
5959.91 & FeI & -2.496 & 4.14 \\
5975.35 & FeI & -0.693 & 4.83 \\
5976.78 & FeI & -1.236 & 3.94 \\
5983.68 & FeI & -0.485 & 4.55 \\
5984.81 & FeI & -0.198 & 4.73 \\
5987.06 & FeI & -0.432 & 4.79 \\
5991.37 & FeII & -3.647 & 3.15 \\
6003.01 & FeI & -1.100 & 3.88 \\
6003.02 & FeI & -6.715 & 5.51 \\
6007.96 & FeI & -0.597 & 4.65 \\
6008.56 & FeI & -0.980 & 3.88 \\
6008.56 & FeI & -7.961 & 2.95 \\
6020.17 & FeI & -0.125 & 4.61 \\
6024.06 & FeI & 0.223 & 4.55 \\
6027.05 & FeI & -1.089 & 4.08 \\
6041.47 & FeI & -1.500 & 5.01 \\
6045.47 & FeII & -2.413 & 6.21 \\
6055.40 & FeI & -1.479 & 4.96 \\
6056.00 & FeI & -0.320 & 4.73 \\
6062.85 & FeI & -3.798 & 2.18 \\
6063.31 & FeI & -0.862 & 4.91 \\
6065.48 & FeI & -1.530 & 2.61 \\
6078.49 & FeI & -0.323 & 4.79 \\
6079.01 & FeI & -1.100 & 4.65 \\
6082.71 & FeI & -3.573 & 2.22 \\
6084.10 & FeII & -3.854 & 3.20 \\
6085.26 & FeI & -2.710 & 2.76 \\
6089.59 & FeI & -3.616 & 4.58 \\
6093.64 & FeI & -1.470 & 4.61 \\
6094.37 & FeI & -1.920 & 4.65 \\
6096.66 & FeI & -1.880 & 3.98 \\
6127.91 & FeI & -1.400 & 4.14 \\
6136.61 & FeI & -1.400 & 2.45 \\
6136.99 & FeI & -2.950 & 2.20 \\
6137.69 & FeI & -1.403 & 2.59 \\
6141.02 & FeII & -5.128 & 3.23 \\
6149.25 & FeII & -2.732 & 3.89 \\
6151.62 & FeI & -3.299 & 2.18 \\
6156.37 & FeI & -3.274 & 3.40 \\
6165.36 & FeI & -1.474 & 4.14 \\
6170.51 & FeI & -0.475 & 4.79 \\
6173.33 & FeI & -2.880 & 2.22 \\
6173.34 & FeI & -4.244 & 5.33 \\
6179.39 & FeII & -2.599 & 5.57 \\
6180.20 & FeI & -2.650 & 2.73 \\
6183.56 & FeI & -1.175 & 5.03 \\
6185.69 & FeI & -0.730 & 5.65 \\
6187.99 & FeI & -1.670 & 3.94 \\
6200.31 & FeI & -2.437 & 2.61 \\
6213.43 & FeI & -2.480 & 2.22 \\
6215.14 & FeI & -1.320 & 4.19 \\
6219.28 & FeI & -2.433 & 2.20 \\
6220.78 & FeI & -2.068 & 3.88 \\
6221.67 & FeI & -5.971 & 0.86 \\
6226.73 & FeI & -1.965 & 3.88 \\
6229.23 & FeI & -2.810 & 2.85 \\
6230.72 & FeI & -1.281 & 2.56 \\
6232.66 & FeI & -5.049 & 5.01 \\
6238.39 & FeII & -2.637 & 3.89 \\
6239.36 & FeII & -4.731 & 2.81 \\
6240.31 & FeI & -1.917 & 4.14 \\
6240.65 & FeI & -3.170 & 2.22 \\
6246.32 & FeI & -0.770 & 3.60 \\
6247.56 & FeII & -2.340 & 3.89 \\
6252.56 & FeI & -1.687 & 2.40 \\
6253.83 & FeI & -1.300 & 4.73 \\
6261.53 & FeI & -0.929 & 5.06 \\
6265.13 & FeI & -2.550 & 2.18 \\
6269.96 & FeII & -4.613 & 3.25 \\
6270.22 & FeI & -2.610 & 2.86 \\
6286.13 & FeI & -0.670 & 5.62 \\
6297.79 & FeI & -2.740 & 2.22 \\
6300.30 & OI & -9.776 & 0.00 \\
6301.50 & FeI & -0.710 & 3.65 \\
6302.49 & FeI & -0.968 & 3.69 \\
6307.52 & FeII & -5.417 & 2.83 \\
6311.50 & FeI & -3.141 & 2.83 \\
6315.81 & FeI & -1.630 & 4.08 \\
6322.69 & FeI & -2.426 & 2.59 \\
6330.85 & FeI & -1.720 & 4.73 \\
6335.33 & FeI & -2.177 & 2.20 \\
6336.82 & FeI & -0.850 & 3.69 \\
6338.88 & FeI & -1.040 & 4.79 \\
6344.15 & FeI & -2.923 & 2.43 \\
6355.03 & FeI & -2.291 & 2.85 \\
6358.70 & FeI & -4.468 & 0.86 \\
6363.78 & OI & -10.258 & 0.02 \\
6369.46 & FeII & -4.291 & 2.89 \\
6380.74 & FeI & -1.376 & 4.19 \\
6383.73 & FeII & -2.275 & 5.55 \\
6385.46 & FeII & -2.663 & 5.55 \\
6392.54 & FeI & -4.526 & 2.28 \\
6393.60 & FeI & -1.580 & 2.43 \\
6400.00 & FeI & -0.270 & 3.60 \\
6400.32 & FeI & -4.318 & 0.92 \\


==> Tables/obslog/obslog.tex <==
OGLE0434 & 2020-11-07T02:47:44.709 & 59160.11649 \\ 
OGLE0434 & 2020-11-07T02:47:52.206 & 59160.11658 \\ 
OGLE0501 & 2020-10-24T04:50:05.197 & 59146.20145 \\ 
OGLE0501 & 2020-10-24T04:50:13.252 & 59146.20154 \\ 
OGLE0512 & 2020-10-24T05:25:26.486 & 59146.22600 \\ 
OGLE0512 & 2020-10-24T05:25:36.488 & 59146.22612 \\ 
OGLE0528 & 2020-10-09T07:28:41.908 & 59131.31160 \\ 
OGLE0528 & 2020-10-09T07:28:48.852 & 59131.31168 \\ 
OGLE0545 & 2020-11-07T03:00:20.624 & 59160.12524 \\ 
OGLE0545 & 2020-11-07T03:00:29.841 & 59160.12535 \\ 
OGLE0590 & 2020-10-26T08:19:13.387 & 59148.34668 \\ 
OGLE0590 & 2020-10-26T08:19:21.279 & 59148.34677 \\ 
OGLE0594 & 2020-10-24T06:09:42.936 & 59146.25675 \\ 
OGLE0594 & 2020-10-24T06:09:49.913 & 59146.25683 \\ 
OGLE0594 & 2020-10-24T06:37:41.388 & 59146.27617 \\ 
OGLE0594 & 2020-10-24T06:37:49.106 & 59146.27626 \\ 
OGLE0648 & 2020-11-07T03:29:44.538 & 59160.14565 \\ 
OGLE0648 & 2020-11-07T03:29:52.365 & 59160.14574 \\ 
OGLE0683 & 2020-11-07T04:07:52.232 & 59160.17213 \\ 
OGLE0683 & 2020-11-07T04:07:59.591 & 59160.17222 \\ 
OGLE0712 & 2020-11-07T04:40:03.399 & 59160.19448 \\ 
OGLE0712 & 2020-11-07T04:40:11.101 & 59160.19457 \\ 
OGLE0716 & 2020-11-09T02:55:21.519 & 59162.12178 \\ 
OGLE0716 & 2020-11-09T02:55:29.431 & 59162.12187 \\ 
OGLE0727 & 2020-11-10T02:20:29.106 & 59163.09756 \\ 
OGLE0727 & 2020-11-10T02:20:36.899 & 59163.09765 \\ 
OGLE0757 & 2020-11-08T07:39:04.532 & 59161.31880 \\ 
OGLE0757 & 2020-11-08T07:39:11.448 & 59161.31888 \\ 
OGLE0757 & 2020-11-08T08:04:12.210 & 59161.33625 \\ 
OGLE0757 & 2020-11-08T08:04:20.535 & 59161.33635 \\ 
OGLE0770 & 2020-11-10T02:46:39.776 & 59163.11574 \\ 
OGLE0770 & 2020-11-10T02:46:47.380 & 59163.11583 \\ 
OGLE0787 & 2020-11-10T06:01:33.654 & 59163.25108 \\ 
OGLE0787 & 2020-11-10T06:01:41.419 & 59163.25117 \\ 
OGLE0798 & 2020-11-09T03:45:06.506 & 59162.15633 \\ 
OGLE0798 & 2020-11-09T03:45:14.930 & 59162.15642 \\ 
OGLE0800 & 2020-11-10T06:29:41.506 & 59163.27062 \\ 
OGLE0800 & 2020-11-10T06:29:48.611 & 59163.27070 \\ 
OGLE0812 & 2020-11-10T07:03:07.455 & 59163.29384 \\ 
OGLE0812 & 2020-11-10T07:03:15.545 & 59163.29393 \\ 
OGLE0819 & 2020-11-10T07:43:40.739 & 59163.32200 \\ 
OGLE0819 & 2020-11-10T07:43:52.080 & 59163.32213 \\ 
OGLE0821 & 2020-11-11T03:48:03.727 & 59164.15838 \\ 
OGLE0821 & 2020-11-11T03:48:12.083 & 59164.15847 \\ 
OGLE0831 & 2020-11-11T04:07:18.368 & 59164.17174 \\ 
OGLE0831 & 2020-11-11T04:07:29.223 & 59164.17187 \\ 
OGLE0844 & 2020-11-11T04:50:47.006 & 59164.20193 \\ 
OGLE0844 & 2020-11-11T04:50:53.984 & 59164.20201 \\ 
OGLE0847 & 2020-11-11T05:15:54.805 & 59164.21938 \\ 
OGLE0847 & 2020-11-11T05:16:01.798 & 59164.21947 \\ 
OGLE0848 & 2020-11-10T08:09:36.138 & 59163.34000 \\ 
OGLE0848 & 2020-11-10T08:09:44.729 & 59163.34010 \\ 
OGLE0888 & 2020-11-09T07:56:53.314 & 59162.33117 \\ 
OGLE0888 & 2020-11-09T07:57:01.486 & 59162.33127 \\ 
OGLE0915 & 2020-11-11T05:49:47.683 & 59164.24291 \\ 
OGLE0915 & 2020-11-11T05:49:54.803 & 59164.24300 \\ 
OGLE0915 & 2020-11-11T06:14:14.760 & 59164.25989 \\ 
OGLE0915 & 2020-11-11T06:14:23.954 & 59164.26000 \\ 
OGLE0936 & 2020-11-11T06:45:04.374 & 59164.28130 \\ 
OGLE0936 & 2020-11-11T06:45:11.371 & 59164.28138 \\ 
OGLE0949 & 2020-11-12T04:02:31.627 & 59165.16842 \\ 
OGLE0949 & 2020-11-12T04:02:39.350 & 59165.16851 \\ 
OGLE0966 & 2020-10-09T06:54:12.669 & 59131.28765 \\ 
OGLE0966 & 2020-10-09T06:54:20.033 & 59131.28773 \\ 
OGLE0969 & 2020-11-11T07:33:38.138 & 59164.31502 \\ 
OGLE0969 & 2020-11-11T07:33:45.430 & 59164.31511 \\ 
OGLE0970 & 2020-11-12T04:37:44.057 & 59165.19287 \\ 
OGLE0970 & 2020-11-12T04:37:51.994 & 59165.19296 \\ 
OGLE0975 & 2020-11-12T05:07:49.280 & 59165.21376 \\ 
OGLE0975 & 2020-11-12T05:07:56.657 & 59165.21385 \\ 
OGLE0978 & 2020-11-12T05:43:29.440 & 59165.23854 \\ 
OGLE0978 & 2020-11-12T05:43:36.373 & 59165.23862 \\ 
OGLE0986 & 2020-11-11T08:11:38.521 & 59164.34142 \\ 
OGLE0986 & 2020-11-11T08:11:47.349 & 59164.34152 \\ 
OGLE0992 & 2020-10-09T07:06:01.942 & 59131.29586 \\ 
OGLE0992 & 2020-10-09T07:06:10.051 & 59131.29595 \\ 
OGLE1001 & 2020-10-09T07:50:15.613 & 59131.32657 \\ 
OGLE1001 & 2020-10-09T07:50:23.258 & 59131.32666 \\ 
OGLE1031 & 2020-10-10T07:28:59.547 & 59132.31180 \\ 
OGLE1031 & 2020-10-10T07:29:06.498 & 59132.31188 \\ 
OGLE1058 & 2020-11-12T06:27:15.380 & 59165.26893 \\ 
OGLE1058 & 2020-11-12T06:27:23.256 & 59165.26902 \\ 
OGLE1080 & 2020-11-12T06:43:42.249 & 59165.28035 \\ 
OGLE1080 & 2020-11-12T06:43:49.212 & 59165.28043 \\ 
OGLE1109 & 2020-11-12T07:09:59.799 & 59165.29861 \\ 
OGLE1109 & 2020-11-12T07:10:08.313 & 59165.29871 \\ 
OGLE1112 & 2020-10-09T08:13:59.599 & 59131.34305 \\ 
OGLE1112 & 2020-10-09T08:14:06.556 & 59131.34313 \\ 
OGLE1313 & 2020-11-13T05:21:20.693 & 59166.22316 \\ 
OGLE1313 & 2020-11-13T05:21:29.103 & 59166.22325 \\ 
OGLE1313 & 2020-11-13T05:45:49.390 & 59166.24015 \\ 
OGLE1313 & 2020-11-13T05:45:58.204 & 59166.24026 \\ 
OGLE1374 & 2020-11-13T06:16:19.724 & 59166.26134 \\ 
OGLE1374 & 2020-11-13T06:16:27.869 & 59166.26143 \\ 
OGLE1374 & 2020-11-13T06:47:09.528 & 59166.28275 \\ 
OGLE1374 & 2020-11-13T06:47:17.066 & 59166.28284 \\ 
OGLE1389 & 2020-11-12T07:43:34.177 & 59165.32192 \\ 
OGLE1389 & 2020-11-12T07:43:45.198 & 59165.32205 \\ 
OGLE1411 & 2020-11-14T04:31:15.249 & 59167.18837 \\ 
OGLE1411 & 2020-11-14T04:31:22.186 & 59167.18845 \\ 
OGLE1411 & 2020-11-14T05:00:24.541 & 59167.20862 \\ 
OGLE1411 & 2020-11-14T05:00:31.543 & 59167.20870 \\ 
OGLE1417 & 2020-11-14T05:36:07.841 & 59167.23342 \\ 
OGLE1417 & 2020-11-14T05:36:18.216 & 59167.23354 \\ 
OGLE1424 & 2020-11-15T06:27:35.742 & 59168.26916 \\ 
OGLE1424 & 2020-11-15T06:27:44.466 & 59168.26926 \\ 
OGLE1424 & 2020-11-15T07:07:14.905 & 59168.29670 \\ 
OGLE1424 & 2020-11-15T07:07:23.692 & 59168.29680 \\ 
OGLE1431 & 2020-11-13T07:22:36.098 & 59166.30736 \\ 
OGLE1431 & 2020-11-13T07:22:43.839 & 59166.30745 \\ 
OGLE1463 & 2020-11-16T04:10:21.074 & 59169.17386 \\ 
OGLE1463 & 2020-11-16T04:10:29.399 & 59169.17395 \\ 
OGLE1463 & 2020-11-16T04:34:10.830 & 59169.19040 \\ 
OGLE1463 & 2020-11-16T04:34:18.574 & 59169.19049 \\ 
OGLE1466 & 2020-11-14T06:23:13.022 & 59167.26612 \\ 
OGLE1466 & 2020-11-14T06:23:19.965 & 59167.26620 \\ 
OGLE1466 & 2020-11-14T07:00:02.432 & 59167.29169 \\ 
OGLE1466 & 2020-11-14T07:00:09.425 & 59167.29178 \\ 
OGLE1490 & 2020-11-17T06:06:55.941 & 59170.25481 \\ 
OGLE1490 & 2020-11-17T06:07:04.005 & 59170.25491 \\ 
OGLE1526 & 2020-11-17T06:48:23.576 & 59170.28361 \\ 
OGLE1526 & 2020-11-17T06:48:31.776 & 59170.28370 \\ 
OGLE1526 & 2020-11-17T07:13:23.492 & 59170.30097 \\ 
OGLE1526 & 2020-11-17T07:13:31.015 & 59170.30105 \\ 
OGLE1539 & 2020-11-17T07:44:06.925 & 59170.32230 \\ 
OGLE1539 & 2020-11-17T07:44:13.896 & 59170.32238 \\ 
OGLE1578 & 2020-11-07T07:53:38.353 & 59160.32892 \\ 
OGLE1578 & 2020-11-07T07:53:45.281 & 59160.32900 \\ 
OGLE1587 & 2020-11-13T08:04:53.644 & 59166.33673 \\ 
OGLE1587 & 2020-11-13T08:05:01.362 & 59166.33682 \\ 
OGLE1616 & 2020-11-15T07:51:39.184 & 59168.32754 \\ 
OGLE1616 & 2020-11-15T07:51:46.194 & 59168.32762 \\ 
OGLE1637 & 2020-10-24T05:11:10.930 & 59146.21610 \\ 
OGLE1637 & 2020-10-24T05:11:19.585 & 59146.21620 \\ 
OGLE1641 & 2020-10-24T05:44:00.477 & 59146.23889 \\ 
OGLE1641 & 2020-10-24T05:44:08.585 & 59146.23899 \\ 
OGLE1647 & 2020-11-14T07:41:41.998 & 59167.32062 \\ 
OGLE1647 & 2020-11-14T07:41:49.422 & 59167.32071 \\ 
OGLE1677 & 2020-11-08T07:18:16.489 & 59161.30436 \\ 
OGLE1677 & 2020-11-08T07:18:24.568 & 59161.30445 \\ 
OGLE1862 & 2020-11-09T06:22:31.686 & 59162.26564 \\ 
OGLE1862 & 2020-11-09T06:22:39.818 & 59162.26574 \\ 
OGLE1939 & 2020-11-07T06:40:06.347 & 59160.27785 \\ 
OGLE1939 & 2020-11-07T06:40:14.688 & 59160.27795 \\ 
OGLE1939 & 2020-11-07T07:14:17.266 & 59160.30159 \\ 
OGLE1939 & 2020-11-07T07:14:24.209 & 59160.30167 \\ 
OGLE1941 & 2020-11-07T05:17:10.861 & 59160.22026 \\ 
OGLE1941 & 2020-11-07T05:17:18.460 & 59160.22035 \\ 
OGLE1941 & 2020-11-07T05:55:57.686 & 59160.24720 \\ 
OGLE1941 & 2020-11-07T05:56:07.369 & 59160.24731 \\ 
OGLE1994 & 2020-11-10T03:46:29.223 & 59163.15728 \\ 
OGLE1994 & 2020-11-10T03:46:36.577 & 59163.15737 \\ 
OGLE2012 & 2020-11-09T07:07:02.917 & 59162.29656 \\ 
OGLE2012 & 2020-11-09T07:07:09.787 & 59162.29664 \\ 
OGLE2019 & 2020-11-10T04:26:44.718 & 59163.18524 \\ 
OGLE2019 & 2020-11-10T04:26:51.980 & 59163.18532 \\ 
OGLE2043 & 2020-11-10T04:46:01.060 & 59163.19862 \\ 
OGLE2043 & 2020-11-10T04:46:09.062 & 59163.19872 \\ 
OGLE2043 & 2020-11-10T05:11:39.588 & 59163.21643 \\ 
OGLE2043 & 2020-11-10T05:11:48.170 & 59163.21653 \\ 
\hline
OGLE0510 & 2000-10-11T04:34:30.713 & 51828.19063 \\ 
OGLE0510 & 2000-10-11T04:44:53.443 & 51828.19784 \\ 


==> Tables/params_abus/Fe_abundances.tex <==
OGLE0434 & -0.40 & 0.12 & 0.07 & 101 & -0.43 & 0.13 & 0.04 & 15 \\ 
OGLE0501 & -0.42 & 0.09 & 0.05 & 84 & -0.43 & 0.06 & 0.03 & 12 \\ 
OGLE0510 & -0.38 & 0.11 & 0.03 & 82 & -0.39 & 0.14 & 0.03 & 9 \\ 
OGLE0512 & -0.48 & 0.13 & 0.06 & 91 & -0.41 & 0.11 & 0.01 & 14 \\ 
OGLE0528 & -0.41 & 0.12 & 0.04 & 91 & -0.43 & 0.07 & 0.02 & 15 \\ 
OGLE0545 & -0.37 & 0.09 & 0.06 & 78 & -0.40 & 0.04 & 0.05 & 10 \\ 
OGLE0590 & -0.41 & 0.10 & 0.23 & 83 & -0.38 & 0.13 & 0.08 & 15 \\ 
OGLE0594 & -0.49 & 0.14 & 0.12 & 71 & -0.50 & 0.02 & 0.10 & 6 \\ 
OGLE0648 & -0.45 & 0.09 & 0.06 & 98 & -0.47 & 0.09 & 0.04 & 17 \\ 
OGLE0683 & -0.38 & 0.11 & 0.07 & 90 & -0.40 & 0.14 & 0.05 & 16 \\ 
OGLE0712 & -0.33 & 0.11 & 0.05 & 101 & -0.34 & 0.11 & 0.05 & 16 \\ 
OGLE0716 & -0.45 & 0.09 & 0.05 & 100 & -0.45 & 0.08 & 0.05 & 14 \\ 
OGLE0727 & -0.55 & 0.09 & 0.17 & 70 & -0.58 & 0.10 & 0.17 & 13 \\ 
OGLE0757 & -0.35 & 0.08 & 0.06 & 75 & -0.34 & 0.11 & 0.05 & 14 \\ 
OGLE0770 & -0.44 & 0.10 & 0.04 & 96 & -0.45 & 0.05 & 0.03 & 14 \\ 
OGLE0787 & -0.38 & 0.16 & 0.05 & 63 & -0.37 & 0.07 & 0.06 & 8 \\ 
OGLE0798 & -0.41 & 0.10 & 0.06 & 82 & -0.45 & 0.08 & 0.05 & 12 \\ 
OGLE0800 & -0.57 & 0.10 & 0.10 & 88 & -0.49 & 0.19 & 0.04 & 15 \\ 
OGLE0812 & -0.39 & 0.11 & 0.07 & 98 & -0.40 & 0.16 & 0.06 & 18 \\ 
OGLE0819 & -0.29 & 0.11 & 0.03 & 85 & -0.29 & 0.06 & 0.02 & 11 \\ 
OGLE0821 & -0.58 & 0.10 & 0.06 & 88 & -0.56 & 0.10 & 0.01 & 14 \\ 
OGLE0831 & -0.40 & 0.10 & 0.05 & 88 & -0.44 & 0.06 & 0.04 & 12 \\ 
OGLE0844 & -0.34 & 0.11 & 0.08 & 82 & -0.33 & 0.12 & 0.07 & 12 \\ 
OGLE0847 & -0.40 & 0.12 & 0.05 & 89 & -0.44 & 0.08 & 0.02 & 14 \\ 
OGLE0848 & -0.46 & 0.08 & 0.10 & 65 & -0.46 & 0.06 & 0.07 & 9 \\ 
OGLE0888 & -0.41 & 0.10 & 0.06 & 100 & -0.45 & 0.12 & 0.04 & 17 \\ 
OGLE0915 & -0.47 & 0.09 & 0.07 & 101 & -0.46 & 0.07 & 0.08 & 14 \\ 
OGLE0936 & -0.49 & 0.11 & 0.04 & 93 & -0.52 & 0.15 & 0.03 & 17 \\ 
OGLE0949 & -0.43 & 0.09 & 0.07 & 83 & -0.43 & 0.08 & 0.06 & 12 \\ 
OGLE0966 & -0.44 & 0.12 & 0.05 & 73 & -0.45 & 0.07 & 0.02 & 9 \\ 
OGLE0969 & -0.38 & 0.11 & 0.04 & 94 & -0.39 & 0.07 & 0.04 & 15 \\ 
OGLE0970 & -0.32 & 0.10 & 0.06 & 82 & -0.34 & 0.10 & 0.04 & 13 \\ 
OGLE0975 & -0.40 & 0.11 & 0.09 & 75 & -0.43 & 0.14 & 0.06 & 14 \\ 
OGLE0978 & -0.43 & 0.10 & 0.04 & 80 & -0.43 & 0.07 & 0.05 & 12 \\ 
OGLE0986 & -0.40 & 0.10 & 0.09 & 69 & -0.45 & 0.16 & 0.08 & 8 \\ 
OGLE0992 & -0.41 & 0.08 & 0.05 & 64 & -0.39 & 0.18 & 0.07 & 7 \\ 
OGLE1001 & -0.31 & 0.12 & 0.05 & 92 & -0.34 & 0.10 & 0.02 & 12 \\ 
OGLE1031 & -0.41 & 0.10 & 0.05 & 69 & -0.43 & 0.09 & 0.02 & 13 \\ 
OGLE1058 & -0.46 & 0.13 & 0.15 & 66 & -0.45 & 0.21 & 0.15 & 14 \\ 
OGLE1080 & -0.49 & 0.16 & 0.08 & 73 & -0.48 & 0.09 & 0.06 & 8 \\ 
OGLE1109 & -0.48 & 0.11 & 0.07 & 90 & -0.50 & 0.07 & 0.06 & 13 \\ 
OGLE1112 & -0.34 & 0.14 & 0.10 & 83 & -0.37 & 0.09 & 0.07 & 12 \\ 
OGLE1313 & -0.79 & 0.09 & 0.13 & 82 & -0.82 & 0.07 & 0.10 & 12 \\ 
OGLE1374 & -0.63 & 0.10 & 0.08 & 75 & -0.67 & 0.09 & 0.08 & 10 \\ 
OGLE1389 & -0.43 & 0.10 & 0.05 & 97 & -0.44 & 0.12 & 0.05 & 15 \\ 
OGLE1411 & -0.49 & 0.11 & 0.07 & 90 & -0.54 & 0.08 & 0.04 & 13 \\ 
OGLE1417 & -0.41 & 0.07 & 0.05 & 70 & -0.44 & 0.05 & 0.03 & 12 \\ 
OGLE1424 & -0.45 & 0.09 & 0.07 & 90 & -0.46 & 0.13 & 0.05 & 14 \\ 
OGLE1431 & -0.33 & 0.08 & 0.06 & 81 & -0.33 & 0.11 & 0.05 & 13 \\ 
OGLE1463 & -0.35 & 0.12 & 0.08 & 86 & -0.41 & 0.11 & 0.03 & 15 \\ 
OGLE1466 & -0.37 & 0.08 & 0.07 & 77 & -0.41 & 0.09 & 0.05 & 13 \\ 
OGLE1490 & -0.53 & 0.11 & 0.07 & 108 & -0.56 & 0.15 & 0.06 & 17 \\ 
OGLE1526 & -0.34 & 0.12 & 0.08 & 89 & -0.37 & 0.11 & 0.05 & 13 \\ 
OGLE1539 & -0.41 & 0.14 & 0.05 & 81 & -0.41 & 0.06 & 0.04 & 14 \\ 
OGLE1578 & -0.30 & 0.11 & 0.06 & 78 & -0.29 & 0.12 & 0.07 & 11 \\ 
OGLE1587 & -0.29 & 0.13 & 0.05 & 68 & -0.32 & 0.03 & 0.02 & 7 \\ 
OGLE1616 & -0.27 & 0.11 & 0.04 & 96 & -0.27 & 0.14 & 0.04 & 16 \\ 
OGLE1637 & -0.35 & 0.12 & 0.08 & 69 & -0.35 & 0.04 & 0.06 & 6 \\ 
OGLE1641 & -0.34 & 0.10 & 0.10 & 89 & -0.37 & 0.15 & 0.07 & 15 \\ 
OGLE1647 & -0.33 & 0.11 & 0.07 & 89 & -0.33 & 0.10 & 0.06 & 14 \\ 
OGLE1677 & -0.31 & 0.12 & 0.08 & 85 & -0.31 & 0.14 & 0.08 & 14 \\ 
OGLE1862 & -0.36 & 0.09 & 0.04 & 85 & -0.34 & 0.09 & 0.06 & 15 \\ 
OGLE1939 & -0.37 & 0.07 & 0.13 & 58 & -0.40 & 0.14 & 0.12 & 13 \\ 
OGLE1941 & -0.22 & 0.09 & 0.06 & 87 & -0.22 & 0.08 & 0.05 & 13 \\ 
OGLE1994 & -0.29 & 0.10 & 0.08 & 93 & -0.32 & 0.14 & 0.06 & 18 \\ 
OGLE2012 & -0.38 & 0.11 & 0.05 & 98 & -0.37 & 0.09 & 0.05 & 14 \\ 
OGLE2019 & -0.13 & 0.15 & 0.06 & 52 & -0.13 & 0.11 & 0.05 & 7 \\ 
OGLE2043 & -0.41 & 0.08 & 0.06 & 86 & -0.41 & 0.09 & 0.05 & 13 \\ 
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\ 


==> Tables/params_abus/O_abundances.tex <==
OGLE0434 & -0.36 & 0.10 & 2 \\ 
OGLE0501 & -0.21 & 0.10 & 2 \\ 
OGLE0510 & -0.30 & 0.06 & 1 \\ 
OGLE0512 & -0.35 & 0.06 & 2 \\ 
OGLE0528 & -0.29 & 0.07 & 2 \\ 
OGLE0545 & -0.22 & 0.10 & 1 \\ 
OGLE0590 & ---- & --- & --- \\ 
OGLE0594 & -0.12 & 0.21 & 1 \\ 
OGLE0648 & -0.32 & 0.11 & 1 \\ 
OGLE0683 & -0.28 & 0.12 & 1 \\ 
OGLE0712 & -0.24 & 0.10 & 2 \\ 
OGLE0716 & -0.24 & 0.09 & 2 \\ 
OGLE0727 & ---- & --- & --- \\ 
OGLE0757 & ---- & --- & --- \\ 
OGLE0770 & -0.47 & 0.10 & 1 \\ 
OGLE0787 & ---- & --- & --- \\ 
OGLE0798 & ---- & --- & --- \\ 
OGLE0800 & ---- & --- & --- \\ 
OGLE0812 & -0.05 & 0.12 & 1 \\ 
OGLE0819 & -0.10 & 0.07 & 1 \\ 
OGLE0821 & -0.43 & 0.08 & 1 \\ 
OGLE0831 & -0.28 & 0.10 & 2 \\ 
OGLE0844 & ---- & --- & --- \\ 
OGLE0847 & -0.29 & 0.09 & 2 \\ 
OGLE0848 & ---- & --- & --- \\ 
OGLE0888 & ---- & --- & --- \\ 
OGLE0915 & -0.36 & 0.13 & 2 \\ 
OGLE0936 & ---- & --- & --- \\ 
OGLE0949 & ---- & --- & --- \\ 
OGLE0966 & -0.42 & 0.05 & 1 \\ 
OGLE0969 & -0.30 & 0.08 & 2 \\ 
OGLE0970 & -0.20 & 0.08 & 1 \\ 
OGLE0975 & ---- & --- & --- \\ 
OGLE0978 & -0.32 & 0.09 & 1 \\ 
OGLE0986 & ---- & --- & --- \\ 
OGLE0992 & -0.32 & 0.11 & 1 \\ 
OGLE1001 & -0.16 & 0.07 & 2 \\ 
OGLE1031 & -0.38 & 0.07 & 1 \\ 
OGLE1058 & 0.04 & 0.27 & 2 \\ 
OGLE1080 & ---- & --- & --- \\ 
OGLE1109 & -0.42 & 0.12 & 1 \\ 
OGLE1112 & 0.19 & 0.13 & 1 \\ 
OGLE1313 & -0.03 & 0.23 & 2 \\ 
OGLE1374 & -0.09 & 0.16 & 1 \\ 
OGLE1389 & -0.40 & 0.10 & 1 \\ 
OGLE1411 & -0.52 & 0.10 & 1 \\ 
OGLE1417 & ---- & --- & --- \\ 
OGLE1424 & ---- & --- & --- \\ 
OGLE1431 & -0.00 & 0.10 & 1 \\ 
OGLE1463 & ---- & --- & --- \\ 
OGLE1466 & -0.24 & 0.09 & 1 \\ 
OGLE1490 & -0.61 & 0.12 & 1 \\ 
OGLE1526 & ---- & --- & --- \\ 
OGLE1539 & -0.08 & 0.09 & 1 \\ 
OGLE1578 & ---- & --- & --- \\ 
OGLE1587 & ---- & --- & --- \\ 
OGLE1616 & -0.22 & 0.08 & 1 \\ 
OGLE1637 & -0.40 & 0.11 & 1 \\ 
OGLE1641 & ---- & --- & --- \\ 
OGLE1647 & ---- & --- & --- \\ 
OGLE1677 & 0.06 & 0.14 & 1 \\ 
OGLE1862 & -0.31 & 0.11 & 1 \\ 
OGLE1939 & ---- & --- & --- \\ 
OGLE1941 & 0.00 & 0.10 & 2 \\ 
OGLE1994 & ---- & --- & --- \\ 
OGLE2012 & -0.31 & 0.10 & 1 \\ 
OGLE2019 & ---- & --- & --- \\ 
OGLE2043 & ---- & --- & --- \\ 


==> Tables/params_abus/parameters.tex <==
OGLE0434 & 5660 & 100 & 0.30 & 0.13 & 2.90 & 0.10 & 0.2577 \\ 
OGLE0501 & 5130 & 77 & 0.30 & 0.05 & 3.10 & 0.09 & 0.4385 \\ 
OGLE0510 & 5530 & 64 & 0.10 & 0.15 & 3.70 & 0.14 & 0.1274 \\ 
OGLE0512 & 5200 & 79 & 0.00 & 0.09 & 3.50 & 0.15 & 0.1892 \\ 
OGLE0528 & 5200 & 64 & 0.10 & 0.08 & 3.50 & 0.19 & 0.3005 \\ 
OGLE0545 & 5420 & 85 & 0.80 & 0.05 & 3.90 & 0.15 & 0.8352 \\ 
OGLE0590 & 5880 & 322 & 0.00 & 0.10 & 3.60 & 0.09 & 0.1314 \\ 
OGLE0594 & 5520 & 194 & 0.90 & 0.05 & 3.60 & 0.23 & 0.6911 \\ 
OGLE0648 & 5300 & 90 & 0.50 & 0.07 & 2.90 & 0.08 & 0.2372 \\ 
OGLE0683 & 5560 & 105 & 0.40 & 0.12 & 3.00 & 0.09 & 0.1281 \\ 
OGLE0712 & 5630 & 77 & 0.50 & 0.10 & 2.90 & 0.09 & 0.3109 \\ 
OGLE0716 & 5130 & 71 & 0.50 & 0.07 & 2.60 & 0.08 & 0.3489 \\ 
OGLE0727 & 5490 & 240 & 0.60 & 0.08 & 4.00 & 0.13 & 0.7902 \\ 
OGLE0757 & 5390 & 100 & 0.90 & 0.08 & 3.70 & 0.13 & 0.5455 \\ 
OGLE0770 & 5130 & 73 & 0.40 & 0.04 & 2.90 & 0.07 & 0.4226 \\ 
OGLE0787 & 4980 & 69 & 0.50 & 0.09 & 4.00 & 0.43 & 0.6923 \\ 
OGLE0798 & 5220 & 83 & 0.70 & 0.07 & 4.00 & 0.18 & 0.5864 \\ 
OGLE0800 & 5830 & 138 & 0.50 & 0.10 & 3.00 & 0.08 & 0.9702 \\ 
OGLE0812 & 6100 & 118 & 0.50 & 0.12 & 2.70 & 0.11 & 0.0206 \\ 
OGLE0819 & 5060 & 55 & 0.70 & 0.06 & 3.40 & 0.16 & 0.4384 \\ 
OGLE0821 & 5160 & 89 & 0.00 & 0.07 & 3.30 & 0.11 & 0.2397 \\ 
OGLE0831 & 5190 & 84 & 0.70 & 0.07 & 3.50 & 0.14 & 0.4606 \\ 
OGLE0844 & 5920 & 141 & 0.40 & 0.13 & 3.40 & 0.14 & 0.1058 \\ 
OGLE0847 & 4930 & 81 & 0.20 & 0.06 & 3.20 & 0.11 & 0.5323 \\ 
OGLE0848 & 5430 & 141 & 0.80 & 0.06 & 3.90 & 0.13 & 0.8285 \\ 
OGLE0888 & 5590 & 87 & 0.60 & 0.10 & 2.80 & 0.07 & 0.9559 \\ 
OGLE0915 & 5430 & 98 & 1.00 & 0.07 & 3.10 & 0.08 & 0.4092 \\ 
OGLE0936 & 5980 & 79 & 0.60 & 0.10 & 3.00 & 0.13 & 0.9814 \\ 
OGLE0949 & 5520 & 95 & 0.80 & 0.06 & 3.90 & 0.17 & 0.8493 \\ 
OGLE0966 & 4900 & 62 & 0.00 & 0.07 & 4.00 & 0.23 & 0.6380 \\ 
OGLE0969 & 5130 & 62 & 0.70 & 0.06 & 3.20 & 0.18 & 0.3468 \\ 
OGLE0970 & 5550 & 80 & 0.50 & 0.08 & 3.40 & 0.12 & 0.1037 \\ 
OGLE0975 & 5690 & 129 & 0.60 & 0.10 & 3.30 & 0.14 & 0.1243 \\ 
OGLE0978 & 5250 & 73 & 0.60 & 0.06 & 3.70 & 0.16 & 0.2940 \\ 
OGLE0986 & 5430 & 132 & 0.10 & 0.15 & 4.00 & 0.16 & 0.9396 \\ 
OGLE0992 & 5370 & 75 & 0.20 & 0.17 & 4.00 & 0.16 & 0.5211 \\ 
OGLE1001 & 5030 & 67 & 0.50 & 0.08 & 3.40 & 0.12 & 0.4434 \\ 
OGLE1031 & 4830 & 59 & 0.40 & 0.06 & 3.70 & 0.13 & 0.5862 \\ 
OGLE1058 & 6060 & 262 & 0.70 & 0.15 & 3.20 & 0.13 & 0.9624 \\ 
OGLE1080 & 5030 & 100 & 0.50 & 0.07 & 4.00 & 0.39 & 0.7434 \\ 
OGLE1109 & 5360 & 100 & 0.80 & 0.06 & 3.60 & 0.14 & 0.6667 \\ 
OGLE1112 & 5620 & 143 & 0.70 & 0.10 & 3.40 & 0.16 & 0.3076 \\ 
OGLE1313 & 6000 & 232 & 0.90 & 0.08 & 3.30 & 0.11 & 0.9292 \\ 
OGLE1374 & 5360 & 143 & 0.60 & 0.09 & 3.70 & 0.16 & 0.3794 \\ 
OGLE1389 & 5530 & 86 & 0.70 & 0.11 & 2.80 & 0.07 & 0.2840 \\ 
OGLE1411 & 5360 & 88 & 0.70 & 0.06 & 3.90 & 0.19 & 0.7261 \\ 
OGLE1417 & 5350 & 74 & 0.70 & 0.05 & 3.90 & 0.12 & 0.4316 \\ 
OGLE1424 & 5730 & 115 & 0.80 & 0.09 & 3.20 & 0.10 & 0.0006 \\ 
OGLE1431 & 5560 & 87 & 0.90 & 0.07 & 3.70 & 0.11 & 0.7531 \\ 
OGLE1463 & 5830 & 119 & 0.50 & 0.10 & 3.00 & 0.09 & 0.1260 \\ 
OGLE1466 & 5720 & 108 & 0.90 & 0.07 & 3.50 & 0.10 & 0.9098 \\ 
OGLE1490 & 5760 & 123 & 0.70 & 0.26 & 2.60 & 0.07 & 0.2465 \\ 
OGLE1526 & 5400 & 114 & 0.90 & 0.09 & 3.90 & 0.14 & 0.7563 \\ 
OGLE1539 & 4970 & 67 & 0.70 & 0.05 & 3.70 & 0.20 & 0.5316 \\ 
OGLE1578 & 5600 & 99 & 1.00 & 0.10 & 3.90 & 0.17 & 0.8202 \\ 
OGLE1587 & 5090 & 63 & 0.60 & 0.05 & 4.00 & 0.31 & 0.6855 \\ 
OGLE1616 & 5420 & 70 & 0.40 & 0.14 & 2.80 & 0.08 & 0.3429 \\ 
OGLE1637 & 5160 & 98 & 0.30 & 0.06 & 4.00 & 0.30 & 0.7816 \\ 
OGLE1641 & 6150 & 152 & 0.40 & 0.12 & 3.20 & 0.12 & 0.0697 \\ 
OGLE1647 & 5790 & 95 & 1.00 & 0.08 & 3.60 & 0.11 & 0.8869 \\ 
OGLE1677 & 6050 & 138 & 0.20 & 0.11 & 3.00 & 0.10 & 0.0333 \\ 
OGLE1862 & 5170 & 65 & 0.60 & 0.07 & 3.10 & 0.10 & 0.2332 \\ 
OGLE1939 & 5550 & 210 & 0.90 & 0.11 & 3.10 & 0.07 & 0.8346 \\ 
OGLE1941 & 5420 & 89 & 1.20 & 0.08 & 3.40 & 0.10 & 0.4380 \\ 
OGLE1994 & 6420 & 137 & 0.90 & 0.11 & 2.80 & 0.08 & 0.9900 \\ 
OGLE2012 & 5660 & 91 & 0.80 & 0.08 & 2.80 & 0.08 & 0.1205 \\ 
OGLE2019 & 5030 & 66 & 0.70 & 0.15 & 4.00 & 0.49 & 0.7111 \\ 
OGLE2043 & 5460 & 99 & 0.80 & 0.07 & 3.10 & 0.08 & 0.3209 \\ 
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\ 


==> Tables/params_abusR08/R08_Fe_abundances.tex <==
OGLE107 & -0.43 & 0.09 & 0.03 & 101 & -0.46 & 0.09 & 0.04 & 17 \\ 
OGLE461 & -0.30 & 0.15 & 0.09 & 65 & -0.30 & 0.08 & 0.10 & 9 \\ 
OGLE655 & -0.41 & 0.11 & 0.06 & 94 & -0.43 & 0.14 & 0.05 & 17 \\ 
OGLE945 & -0.53 & 0.09 & 0.04 & 83 & -0.47 & 0.09 & 0.00 & 14 \\ 
OGLE1100 & -0.33 & 0.12 & 0.07 & 79 & -0.35 & 0.19 & 0.04 & 18 \\ 
OGLE1128 & -0.51 & 0.12 & 0.04 & 82 & -0.51 & 0.10 & 0.05 & 13 \\ 
OGLE1290 & -0.37 & 0.13 & 0.05 & 59 & -0.36 & 0.07 & 0.04 & 7 \\ 
OGLE1327 & -0.50 & 0.15 & 0.08 & 81 & -0.52 & 0.10 & 0.06 & 13 \\ 
OGLE2337 & -0.36 & 0.09 & 0.04 & 87 & -0.36 & 0.11 & 0.04 & 15 \\ 
OGLE2832 & -0.28 & 0.15 & 0.12 & 63 & -0.30 & 0.10 & 0.12 & 9 \\ 
OGLE2949 & -0.44 & 0.11 & 0.03 & 88 & -0.45 & 0.10 & 0.05 & 15 \\ 
OGLE3158 & -0.45 & 0.09 & 0.06 & 78 & -0.44 & 0.13 & 0.06 & 14 \\ 
OGLE3320 & -0.40 & 0.12 & 0.05 & 75 & -0.41 & 0.13 & 0.06 & 9 \\ 
OGLE4033 & -0.78 & 0.09 & 0.04 & 97 & -0.76 & 0.09 & 0.04 & 16 \\ 
OGLE4061 & -0.44 & 0.09 & 0.03 & 89 & -0.46 & 0.09 & 0.02 & 15 \\ 
OGLE4208 & -0.55 & 0.09 & 0.03 & 80 & -0.56 & 0.09 & 0.02 & 14 \\ 
OGLE4357 & -0.47 & 0.08 & 0.04 & 89 & -0.46 & 0.07 & 0.04 & 15 \\ 
OGLE4451 & -0.51 & 0.10 & 0.07 & 90 & -0.51 & 0.10 & 0.09 & 16 \\ 
OGLE4544 & -0.44 & 0.07 & 0.03 & 77 & -0.44 & 0.08 & 0.02 & 12 \\ 
OGLE4628 & -0.53 & 0.10 & 0.07 & 67 & -0.32 & 0.16 & -0.02 & 9 \\ 
OGLE4689 & -0.40 & 0.12 & 0.08 & 68 & -0.38 & 0.06 & 0.02 & 7 \\ 


==> Tables/params_abusR08/R08_O_abundances.tex <==
OGLE107 & -0.33 & 0.06 & 2 \\ 
OGLE461 & 0.03 & 0.18 & 2 \\ 
OGLE655 & -0.28 & 0.10 & 1 \\ 
OGLE945 & -0.38 & 0.03 & 2 \\ 
OGLE1100 & 0.02 & 0.10 & 2 \\ 
OGLE1128 & -0.33 & 0.09 & 1 \\ 
OGLE1290 & -0.29 & 0.07 & 1 \\ 
OGLE1327 & -0.17 & 0.12 & 1 \\ 
OGLE2337 & -0.33 & 0.07 & 1 \\ 
OGLE2832 & ---- & --- & --- \\ 
OGLE2949 & -0.37 & 0.08 & 1 \\ 
OGLE3158 & ---- & --- & --- \\ 
OGLE3320 & 0.43 & 0.10 & 1 \\ 
OGLE4033 & ---- & --- & --- \\ 
OGLE4061 & -0.44 & 0.07 & 1 \\ 
OGLE4208 & -0.37 & 0.04 & 1 \\ 
OGLE4357 & -0.40 & 0.07 & 1 \\ 
OGLE4451 & -0.29 & 0.12 & 1 \\ 
OGLE4544 & -0.43 & 0.05 & 1 \\ 
OGLE4628 & -0.34 & 0.02 & 1 \\ 
OGLE4689 & -0.29 & 0.07 & 1 \\ 


==> Tables/params_abusR08/R08_parameters.tex <==
OGLE107 & 5390 & 42 & 0.80 & 0.07 & 2.80 & 0.06 & 0.860 \\ 
OGLE461 & 4890 & 109 & 0.70 & 0.08 & 4.00 & 0.51 & 0.682 \\ 
OGLE655 & 5590 & 86 & 0.50 & 0.11 & 3.20 & 0.11 & 0.144 \\ 
OGLE945 & 4960 & 40 & 0.00 & 0.09 & 3.60 & 0.12 & 0.605 \\ 
OGLE1100 & 6200 & 122 & 0.70 & 0.16 & 3.10 & 0.17 & 0.201 \\ 
OGLE1128 & 5370 & 65 & 0.80 & 0.09 & 3.70 & 0.19 & 0.861 \\ 
OGLE1290 & 4870 & 64 & 0.10 & 0.08 & 4.00 & 1.04 & 0.136 \\ 
OGLE1327 & 5660 & 122 & 0.70 & 0.09 & 3.20 & 0.16 & 0.037 \\ 
OGLE2337 & 5590 & 56 & 0.40 & 0.09 & 3.20 & 0.12 & 0.130 \\ 
OGLE2832 & 5060 & 164 & 0.80 & 0.10 & 4.00 & 0.63 & 0.710 \\ 
OGLE2949 & 5230 & 51 & 0.20 & 0.11 & 3.20 & 0.12 & 0.917 \\ 
OGLE3158 & 5630 & 108 & 0.20 & 0.10 & 3.40 & 0.14 & 0.144 \\ 
OGLE3320 & 5880 & 87 & 1.40 & 0.15 & 3.70 & 0.20 & 0.024 \\ 
OGLE4033 & 5500 & 72 & 0.60 & 0.09 & 2.60 & 0.08 & 0.237 \\ 
OGLE4061 & 5230 & 49 & 0.20 & 0.08 & 3.00 & 0.08 & 0.119 \\ 
OGLE4208 & 5290 & 38 & 0.80 & 0.08 & 3.60 & 0.12 & 0.411 \\ 
OGLE4357 & 5290 & 47 & 0.20 & 0.07 & 3.40 & 0.12 & 0.059 \\ 
OGLE4451 & 5530 & 92 & 0.70 & 0.10 & 3.00 & 0.09 & 0.055 \\ 
OGLE4544 & 5330 & 36 & 0.70 & 0.08 & 3.20 & 0.11 & 0.342 \\ 
OGLE4628 & 4900 & 65 & 0.00 & 0.13 & 4.00 & 0.23 & 0.321 \\ 
OGLE4689 & 4840 & 94 & 0.00 & 0.07 & 4.00 & 0.23 & 0.880 \\ 

